Is 4 Bits Enough for EEG Sleep Staging? A Subject-Level Benchmark of MXFP4, NVFP4 and FP8

Staging sleep on a wearable device keeps the raw electroencephalogram (EEG) private and saves the energy needed to transmit it. It also requires small, energy-efficient neural networks. We benchmark 13 post-training quantization (PTQ) configurations, from FP16 to the block-scaled 4-bit formats MXFP4 and NVFP4, for five-stage sleep staging from single-channel Fpz-Cz EEG. We use Sleep-EDF-78 (78 subjects), subject-wise cross-validation, three training seeds, value-exact emulation, and per-subject paired statistics. All 8- and 16-bit formats stay within 0.45 percentage points (pp) of FP32 Macro-F1. With 4-bit weights and activations, an epoch-wise CNN loses 1.98 to 3.04 pp, and a temporal-context network loses at most 1.19 pp. A same-encoder ablation shows that temporal context explains little of this gap. At equal block size, NVFP4 outperforms MXFP4. The first layer, which quantizes the raw EEG, is the most sensitive layer in both networks. Keeping the first and last layers in FP8 brings both tested 4-bit formats within 0.48 pp of FP32. This recipe adds at most 2.1% weight storage, needs no retraining, and is equivalent to quantization-aware training (QAT) within an exploratory 1-pp margin. The 4-bit losses fall on the same subjects across architectures (Spearman correlation coefficient = 0.69 to 0.79), and they reduce N3 recall the most. On the nested Sleep-EDF-20 subset, NVFP4 with FP8 first and last layers again stays within 0.25 pp of FP32. Under MXFP4, however, the ranking of the architectures reverses, and FP8 first and last layers do not fully recover two of the three tested models. In our emulation, NVFP4 with FP8 first and last layers thus loses little accuracy without QAT in both cohorts.

==> numbers.tex <==
% AUTO-GENERATED by make_numbers.py from the validated notebook outputs. Do not edit by hand.
\providecommand{\mns}{\ensuremath{-}}\providecommand{\pls}{\ensuremath{+}}
\makeatletter
\newcommand{\val}[1]{\ifcsname v@#1\endcsname\csname v@#1\endcsname\else\textbf{??#1??}\PackageWarning{numbers}{UNDEFINED VALUE #1}\fi}
\expandafter\def\csname v@abl.cnn.fp32.acc\endcsname{74.7}
\expandafter\def\csname v@abl.cnn.fp32.kappa\endcsname{0.661}
\expandafter\def\csname v@abl.cnn.fp32.mf1\endcsname{69.9}
\expandafter\def\csname v@abl.cnn.fp32.mf1sd\endcsname{0.26}
\expandafter\def\csname v@abl.cnn.mxfp416w4a4.d\endcsname{\mns{}3.02}
\expandafter\def\csname v@abl.cnn.mxfp416w4a4.hi\endcsname{\mns{}2.26}
\expandafter\def\csname v@abl.cnn.mxfp416w4a4.lo\endcsname{\mns{}3.77}
\expandafter\def\csname v@abl.cnn.mxfp416w4a4.med\endcsname{\mns{}2.47}
\expandafter\def\csname v@abl.cnn.mxfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4.d\endcsname{\mns{}3.04}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4.hi\endcsname{\mns{}2.31}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4.lo\endcsname{\mns{}3.77}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4.med\endcsname{\mns{}2.14}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.48}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4fp8firstlast.hi\endcsname{\mns{}0.34}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.61}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.38}
\expandafter\def\csname v@abl.cnn.mxfp432w4a4fp8firstlast.p\endcsname{<0.001}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4.d\endcsname{\mns{}1.98}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4.hi\endcsname{\mns{}1.42}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4.lo\endcsname{\mns{}2.55}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4.med\endcsname{\mns{}1.62}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4fp8firstlast.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4fp8firstlast.hi\endcsname{\mns{}0.13}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.36}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4fp8firstlast.med\endcsname{\mns{}0.18}
\expandafter\def\csname v@abl.cnn.nvfp416w4a4fp8firstlast.p\endcsname{<0.001}
\expandafter\def\csname v@abl.cnn.nvfp432w4a4.d\endcsname{\mns{}2.38}
\expandafter\def\csname v@abl.cnn.nvfp432w4a4.hi\endcsname{\mns{}1.76}
\expandafter\def\csname v@abl.cnn.nvfp432w4a4.lo\endcsname{\mns{}3.04}
\expandafter\def\csname v@abl.cnn.nvfp432w4a4.med\endcsname{\mns{}1.92}
\expandafter\def\csname v@abl.cnn.nvfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.mxfp416w4a4.d\endcsname{\pls{}1.28}
\expandafter\def\csname v@abl.con.enc.mxfp416w4a4.hi\endcsname{\pls{}1.84}
\expandafter\def\csname v@abl.con.enc.mxfp416w4a4.lo\endcsname{\pls{}0.70}
\expandafter\def\csname v@abl.con.enc.mxfp416w4a4.med\endcsname{\pls{}1.38}
\expandafter\def\csname v@abl.con.enc.mxfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.mxfp416w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4.d\endcsname{\pls{}1.58}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4.hi\endcsname{\pls{}2.13}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4.lo\endcsname{\pls{}1.05}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4.med\endcsname{\pls{}1.34}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4fp8firstlast.d\endcsname{\pls{}0.20}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.40}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.01}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4fp8firstlast.med\endcsname{\pls{}0.25}
\expandafter\def\csname v@abl.con.enc.mxfp432w4a4fp8firstlast.p\endcsname{0.01}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4.d\endcsname{\pls{}1.31}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4.hi\endcsname{\pls{}1.72}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4.lo\endcsname{\pls{}0.92}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4.med\endcsname{\pls{}1.19}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.28}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.44}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4fp8firstlast.lo\endcsname{\pls{}0.13}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.22}
\expandafter\def\csname v@abl.con.enc.nvfp416w4a4fp8firstlast.p\endcsname{0.002}
\expandafter\def\csname v@abl.con.enc.nvfp432w4a4.d\endcsname{\pls{}1.59}
\expandafter\def\csname v@abl.con.enc.nvfp432w4a4.hi\endcsname{\pls{}1.96}
\expandafter\def\csname v@abl.con.enc.nvfp432w4a4.lo\endcsname{\pls{}1.22}
\expandafter\def\csname v@abl.con.enc.nvfp432w4a4.med\endcsname{\pls{}1.63}
\expandafter\def\csname v@abl.con.enc.nvfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@abl.con.enc.nvfp432w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@abl.con.tcn.mxfp416w4a4.d\endcsname{\pls{}0.54}
\expandafter\def\csname v@abl.con.tcn.mxfp416w4a4.hi\endcsname{\pls{}1.16}
\expandafter\def\csname v@abl.con.tcn.mxfp416w4a4.lo\endcsname{\mns{}0.04}
\expandafter\def\csname v@abl.con.tcn.mxfp416w4a4.med\endcsname{\mns{}0.07}
\expandafter\def\csname v@abl.con.tcn.mxfp416w4a4.p\endcsname{0.38}
\expandafter\def\csname v@abl.con.tcn.mxfp416w4a4.ph\endcsname{1.00}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4.d\endcsname{\pls{}0.55}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4.hi\endcsname{\pls{}1.10}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4.lo\endcsname{\pls{}0.01}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4.med\endcsname{\pls{}0.05}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4.p\endcsname{0.37}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4.ph\endcsname{1.00}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4fp8firstlast.d\endcsname{\pls{}0.14}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.39}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.11}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4fp8firstlast.med\endcsname{\pls{}0.09}
\expandafter\def\csname v@abl.con.tcn.mxfp432w4a4fp8firstlast.p\endcsname{0.14}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4.d\endcsname{\pls{}0.18}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4.hi\endcsname{\pls{}0.54}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4.lo\endcsname{\mns{}0.18}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4.med\endcsname{\pls{}0.07}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4.p\endcsname{0.48}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4.ph\endcsname{1.00}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.15}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.11}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.01}
\expandafter\def\csname v@abl.con.tcn.nvfp416w4a4fp8firstlast.p\endcsname{0.97}
\expandafter\def\csname v@abl.con.tcn.nvfp432w4a4.d\endcsname{\pls{}0.40}
\expandafter\def\csname v@abl.con.tcn.nvfp432w4a4.hi\endcsname{\pls{}0.78}
\expandafter\def\csname v@abl.con.tcn.nvfp432w4a4.lo\endcsname{\pls{}0.04}
\expandafter\def\csname v@abl.con.tcn.nvfp432w4a4.med\endcsname{\pls{}0.23}
\expandafter\def\csname v@abl.con.tcn.nvfp432w4a4.p\endcsname{0.07}
\expandafter\def\csname v@abl.con.tcn.nvfp432w4a4.ph\endcsname{0.28}
\expandafter\def\csname v@abl.ctx.fp32.acc\endcsname{79.9}
\expandafter\def\csname v@abl.ctx.fp32.kappa\endcsname{0.731}
\expandafter\def\csname v@abl.ctx.fp32.mf1\endcsname{75.6}
\expandafter\def\csname v@abl.ctx.fp32.mf1sd\endcsname{0.81}
\expandafter\def\csname v@abl.ctx.mxfp416w4a4.d\endcsname{\mns{}1.19}
\expandafter\def\csname v@abl.ctx.mxfp416w4a4.hi\endcsname{\mns{}0.52}
\expandafter\def\csname v@abl.ctx.mxfp416w4a4.lo\endcsname{\mns{}1.92}
\expandafter\def\csname v@abl.ctx.mxfp416w4a4.med\endcsname{\mns{}0.63}
\expandafter\def\csname v@abl.ctx.mxfp416w4a4.p\endcsname{0.004}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4.d\endcsname{\mns{}0.91}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4.hi\endcsname{\mns{}0.30}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4.lo\endcsname{\mns{}1.55}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4.med\endcsname{\mns{}0.53}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4.p\endcsname{0.02}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.13}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.11}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.40}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4fp8firstlast.med\endcsname{\pls{}0.04}
\expandafter\def\csname v@abl.ctx.mxfp432w4a4fp8firstlast.p\endcsname{0.96}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4.d\endcsname{\mns{}0.49}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4.hi\endcsname{\mns{}0.05}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4.lo\endcsname{\mns{}0.93}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4.med\endcsname{\mns{}0.25}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4.p\endcsname{0.07}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.06}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.15}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.04}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.11}
\expandafter\def\csname v@abl.ctx.nvfp416w4a4fp8firstlast.p\endcsname{0.07}
\expandafter\def\csname v@abl.ctx.nvfp432w4a4.d\endcsname{\mns{}0.39}
\expandafter\def\csname v@abl.ctx.nvfp432w4a4.hi\endcsname{\pls{}0.09}
\expandafter\def\csname v@abl.ctx.nvfp432w4a4.lo\endcsname{\mns{}0.88}
\expandafter\def\csname v@abl.ctx.nvfp432w4a4.med\endcsname{\mns{}0.08}
\expandafter\def\csname v@abl.ctx.nvfp432w4a4.p\endcsname{0.29}
\expandafter\def\csname v@abl.enc.fp32.acc\endcsname{74.0}
\expandafter\def\csname v@abl.enc.fp32.kappa\endcsname{0.653}
\expandafter\def\csname v@abl.enc.fp32.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.enc.fp32.mf1sd\endcsname{0.64}
\expandafter\def\csname v@abl.enc.mxfp416w4a4.d\endcsname{\mns{}1.74}
\expandafter\def\csname v@abl.enc.mxfp416w4a4.hi\endcsname{\mns{}0.79}
\expandafter\def\csname v@abl.enc.mxfp416w4a4.lo\endcsname{\mns{}2.72}
\expandafter\def\csname v@abl.enc.mxfp416w4a4.med\endcsname{\mns{}0.91}
\expandafter\def\csname v@abl.enc.mxfp416w4a4.p\endcsname{0.006}
\expandafter\def\csname v@abl.enc.mxfp432w4a4.d\endcsname{\mns{}1.46}
\expandafter\def\csname v@abl.enc.mxfp432w4a4.hi\endcsname{\mns{}0.61}
\expandafter\def\csname v@abl.enc.mxfp432w4a4.lo\endcsname{\mns{}2.34}
\expandafter\def\csname v@abl.enc.mxfp432w4a4.med\endcsname{\mns{}0.67}
\expandafter\def\csname v@abl.enc.mxfp432w4a4.p\endcsname{0.01}
\expandafter\def\csname v@abl.enc.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.28}
\expandafter\def\csname v@abl.enc.mxfp432w4a4fp8firstlast.hi\endcsname{\mns{}0.06}
\expandafter\def\csname v@abl.enc.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.49}
\expandafter\def\csname v@abl.enc.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.13}
\expandafter\def\csname v@abl.enc.mxfp432w4a4fp8firstlast.p\endcsname{0.02}
\expandafter\def\csname v@abl.enc.nvfp416w4a4.d\endcsname{\mns{}0.66}
\expandafter\def\csname v@abl.enc.nvfp416w4a4.hi\endcsname{\mns{}0.14}
\expandafter\def\csname v@abl.enc.nvfp416w4a4.lo\endcsname{\mns{}1.22}
\expandafter\def\csname v@abl.enc.nvfp416w4a4.med\endcsname{\mns{}0.38}
\expandafter\def\csname v@abl.enc.nvfp416w4a4.p\endcsname{0.05}
\expandafter\def\csname v@abl.enc.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.04}
\expandafter\def\csname v@abl.enc.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.15}
\expandafter\def\csname v@abl.enc.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.08}
\expandafter\def\csname v@abl.enc.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.06}
\expandafter\def\csname v@abl.enc.nvfp416w4a4fp8firstlast.p\endcsname{0.28}
\expandafter\def\csname v@abl.enc.nvfp432w4a4.d\endcsname{\mns{}0.79}
\expandafter\def\csname v@abl.enc.nvfp432w4a4.hi\endcsname{\mns{}0.24}
\expandafter\def\csname v@abl.enc.nvfp432w4a4.lo\endcsname{\mns{}1.36}
\expandafter\def\csname v@abl.enc.nvfp432w4a4.med\endcsname{\mns{}0.24}
\expandafter\def\csname v@abl.enc.nvfp432w4a4.p\endcsname{0.03}
\expandafter\def\csname v@abl.enc.phmax\endcsname{<0.001}
\expandafter\def\csname v@abl.enc.rmax\endcsname{\pls{}1.59}
\expandafter\def\csname v@abl.enc.rmin\endcsname{\pls{}1.28}
\expandafter\def\csname v@abl.enc.wfour.max\endcsname{1.74}
\expandafter\def\csname v@abl.enc.wfour.min\endcsname{0.66}
\expandafter\def\csname v@abl.encmain.bf16.d\endcsname{\mns{}0.00}
\expandafter\def\csname v@abl.encmain.bf16.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@abl.encmain.bf16.lo\endcsname{\mns{}0.01}
\expandafter\def\csname v@abl.encmain.bf16.med\endcsname{\mns{}0.01}
\expandafter\def\csname v@abl.encmain.bf16.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.bf16.p\endcsname{0.56}
\expandafter\def\csname v@abl.encmain.bf16.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.fp16.d\endcsname{\mns{}0.00}
\expandafter\def\csname v@abl.encmain.fp16.hi\endcsname{\pls{}0.00}
\expandafter\def\csname v@abl.encmain.fp16.lo\endcsname{\mns{}0.01}
\expandafter\def\csname v@abl.encmain.fp16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@abl.encmain.fp16.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.fp16.p\endcsname{0.64}
\expandafter\def\csname v@abl.encmain.fp16.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.d\endcsname{\mns{}0.04}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.lo\endcsname{\mns{}0.11}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.p\endcsname{0.48}
\expandafter\def\csname v@abl.encmain.fp8e4m3w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.d\endcsname{\pls{}0.04}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.hi\endcsname{\pls{}0.21}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.lo\endcsname{\mns{}0.14}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.med\endcsname{\pls{}0.22}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.mf1\endcsname{69.1}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.p\endcsname{0.32}
\expandafter\def\csname v@abl.encmain.fp8e5m2w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.int4g32w4.d\endcsname{\mns{}0.26}
\expandafter\def\csname v@abl.encmain.int4g32w4.hi\endcsname{\mns{}0.11}
\expandafter\def\csname v@abl.encmain.int4g32w4.lo\endcsname{\mns{}0.42}
\expandafter\def\csname v@abl.encmain.int4g32w4.med\endcsname{\mns{}0.19}
\expandafter\def\csname v@abl.encmain.int4g32w4.mf1\endcsname{68.7}
\expandafter\def\csname v@abl.encmain.int4g32w4.p\endcsname{0.002}
\expandafter\def\csname v@abl.encmain.int4g32w4.ph\endcsname{0.03}
\expandafter\def\csname v@abl.encmain.int8w8.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@abl.encmain.int8w8.hi\endcsname{\pls{}0.00}
\expandafter\def\csname v@abl.encmain.int8w8.lo\endcsname{\mns{}0.05}
\expandafter\def\csname v@abl.encmain.int8w8.med\endcsname{\mns{}0.01}
\expandafter\def\csname v@abl.encmain.int8w8.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.int8w8.p\endcsname{0.08}
\expandafter\def\csname v@abl.encmain.int8w8.ph\endcsname{0.77}
\expandafter\def\csname v@abl.encmain.int8w8a8.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@abl.encmain.int8w8a8.hi\endcsname{\pls{}0.03}
\expandafter\def\csname v@abl.encmain.int8w8a8.lo\endcsname{\mns{}0.07}
\expandafter\def\csname v@abl.encmain.int8w8a8.med\endcsname{\mns{}0.02}
\expandafter\def\csname v@abl.encmain.int8w8a8.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.int8w8a8.p\endcsname{0.78}
\expandafter\def\csname v@abl.encmain.int8w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.d\endcsname{\mns{}1.74}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.hi\endcsname{\mns{}0.79}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.lo\endcsname{\mns{}2.72}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.med\endcsname{\mns{}0.91}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.mf1\endcsname{68.3}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.p\endcsname{0.006}
\expandafter\def\csname v@abl.encmain.mxfp416w4a4.ph\endcsname{0.09}
\expandafter\def\csname v@abl.encmain.mxfp432w4.d\endcsname{\mns{}0.44}
\expandafter\def\csname v@abl.encmain.mxfp432w4.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@abl.encmain.mxfp432w4.lo\endcsname{\mns{}0.91}
\expandafter\def\csname v@abl.encmain.mxfp432w4.med\endcsname{\mns{}0.00}
\expandafter\def\csname v@abl.encmain.mxfp432w4.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.mxfp432w4.p\endcsname{0.24}
\expandafter\def\csname v@abl.encmain.mxfp432w4.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.d\endcsname{\mns{}1.46}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.hi\endcsname{\mns{}0.61}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.lo\endcsname{\mns{}2.34}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.med\endcsname{\mns{}0.67}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.mf1\endcsname{68.5}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.p\endcsname{0.01}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4.ph\endcsname{0.15}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.d\endcsname{\mns{}0.41}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.hi\endcsname{\mns{}0.20}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.lo\endcsname{\mns{}0.62}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.med\endcsname{\mns{}0.35}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.mf1\endcsname{68.8}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.p\endcsname{<0.001}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8first.ph\endcsname{0.01}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.28}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.hi\endcsname{\mns{}0.06}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.49}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.13}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.p\endcsname{0.02}
\expandafter\def\csname v@abl.encmain.mxfp432w4a4fp8firstlast.ph\endcsname{0.29}
\expandafter\def\csname v@abl.encmain.nvfp416w4.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@abl.encmain.nvfp416w4.hi\endcsname{\mns{}0.01}
\expandafter\def\csname v@abl.encmain.nvfp416w4.lo\endcsname{\mns{}0.49}
\expandafter\def\csname v@abl.encmain.nvfp416w4.med\endcsname{\mns{}0.10}
\expandafter\def\csname v@abl.encmain.nvfp416w4.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.nvfp416w4.p\endcsname{0.10}
\expandafter\def\csname v@abl.encmain.nvfp416w4.ph\endcsname{0.89}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.d\endcsname{\mns{}0.66}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.hi\endcsname{\mns{}0.14}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.lo\endcsname{\mns{}1.22}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.med\endcsname{\mns{}0.38}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.mf1\endcsname{68.8}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.p\endcsname{0.05}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4.ph\endcsname{0.58}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.d\endcsname{\mns{}0.07}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.hi\endcsname{\pls{}0.10}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.lo\endcsname{\mns{}0.24}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.med\endcsname{\mns{}0.06}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.mf1\endcsname{68.9}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.p\endcsname{0.49}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8first.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.04}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.15}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.08}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.06}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.mf1\endcsname{69.0}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.p\endcsname{0.28}
\expandafter\def\csname v@abl.encmain.nvfp416w4a4fp8firstlast.ph\endcsname{1.00}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.d\endcsname{\mns{}0.79}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.hi\endcsname{\mns{}0.24}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.lo\endcsname{\mns{}1.36}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.med\endcsname{\mns{}0.24}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.mf1\endcsname{68.8}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.p\endcsname{0.03}
\expandafter\def\csname v@abl.encmain.nvfp432w4a4.ph\endcsname{0.35}
\expandafter\def\csname v@abl.rho.max\endcsname{0.79}
\expandafter\def\csname v@abl.rho.min\endcsname{0.74}
\expandafter\def\csname v@abl.tcn.phmin\endcsname{0.28}
\expandafter\def\csname v@abl.tcn.rmax\endcsname{\pls{}0.55}
\expandafter\def\csname v@abl.tcn.rmin\endcsname{\pls{}0.18}
\expandafter\def\csname v@cal.distmax\endcsname{28{,}535}
\expandafter\def\csname v@cal.distmin\endcsname{27{,}828}
\expandafter\def\csname v@cal.nI\endcsname{13.1}
\expandafter\def\csname v@cal.nII\endcsname{30.5}
\expandafter\def\csname v@cal.positions\endcsname{31{,}620}
\expandafter\def\csname v@cm.cnn.mx.abs.nIIInII\endcsname{923}
\expandafter\def\csname v@cm.cnn.mx.abs.nIInI\endcsname{5{,}884}
\expandafter\def\csname v@cm.cnn.nv.abs.nIIInII\endcsname{705}
\expandafter\def\csname v@cm.cnn.nv.abs.nIInI\endcsname{3{,}675}
\expandafter\def\csname v@cm.ctx.mx.abs.nIIInII\endcsname{1{,}161}
\expandafter\def\csname v@cm.ctx.mx.abs.nIInI\endcsname{1{,}462}
\expandafter\def\csname v@cm.ctx.nv.abs.nIIInII\endcsname{593}
\expandafter\def\csname v@cm.ctx.nv.abs.nIInI\endcsname{1{,}778}
\expandafter\def\csname v@cnn.bf16.acc\endcsname{74.7}
\expandafter\def\csname v@cnn.bf16.actkib\endcsname{24.3}
\expandafter\def\csname v@cnn.bf16.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@cnn.bf16.dabs\endcsname{0.01}
\expandafter\def\csname v@cnn.bf16.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@cnn.bf16.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@cnn.bf16.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.bf16.f1n2\endcsname{78.4}
\expandafter\def\csname v@cnn.bf16.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.bf16.f1rem\endcsname{64.8}
\expandafter\def\csname v@cnn.bf16.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.bf16.flip\endcsname{0.1}
\expandafter\def\csname v@cnn.bf16.gbops\endcsname{0.266}
\expandafter\def\csname v@cnn.bf16.kappa\endcsname{0.661}
\expandafter\def\csname v@cnn.bf16.kib\endcsname{108.5}
\expandafter\def\csname v@cnn.bf16.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.bf16.lttwo\endcsname{0.0}
\expandafter\def\csname v@cnn.bf16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@cnn.bf16.mf1\endcsname{69.9}
\expandafter\def\csname v@cnn.bf16.mf1sd\endcsname{0.25}
\expandafter\def\csname v@cnn.bf16.n\endcsname{234}
\expandafter\def\csname v@cnn.bf16.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.bf16.p\endcsname{0.38}
\expandafter\def\csname v@cnn.bf16.pfive\endcsname{\mns{}0.17}
\expandafter\def\csname v@cnn.bf16.ph\endcsname{1.00}
\expandafter\def\csname v@cnn.bf16.tflip\endcsname{0.1}
\expandafter\def\csname v@cnn.budget\endcsname{30}
\expandafter\def\csname v@cnn.epmed\endcsname{11}
\expandafter\def\csname v@cnn.firstmacpct\endcsname{45.5}
\expandafter\def\csname v@cnn.fp16.acc\endcsname{74.7}
\expandafter\def\csname v@cnn.fp16.actkib\endcsname{24.3}
\expandafter\def\csname v@cnn.fp16.compr\endcsname{2.0}
\expandafter\def\csname v@cnn.fp16.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@cnn.fp16.dabs\endcsname{0.00}
\expandafter\def\csname v@cnn.fp16.dhi\endcsname{\pls{}0.00}
\expandafter\def\csname v@cnn.fp16.dlo\endcsname{\mns{}0.00}
\expandafter\def\csname v@cnn.fp16.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.fp16.f1n2\endcsname{78.4}
\expandafter\def\csname v@cnn.fp16.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.fp16.f1rem\endcsname{64.9}
\expandafter\def\csname v@cnn.fp16.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.fp16.flip\endcsname{0.0}
\expandafter\def\csname v@cnn.fp16.gbops\endcsname{0.266}
\expandafter\def\csname v@cnn.fp16.kappa\endcsname{0.662}
\expandafter\def\csname v@cnn.fp16.kib\endcsname{108.5}
\expandafter\def\csname v@cnn.fp16.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.fp16.lttwo\endcsname{0.0}
\expandafter\def\csname v@cnn.fp16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@cnn.fp16.mf1\endcsname{69.9}
\expandafter\def\csname v@cnn.fp16.mf1sd\endcsname{0.26}
\expandafter\def\csname v@cnn.fp16.n\endcsname{234}
\expandafter\def\csname v@cnn.fp16.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.fp16.p\endcsname{0.68}
\expandafter\def\csname v@cnn.fp16.pfive\endcsname{\mns{}0.04}
\expandafter\def\csname v@cnn.fp16.ph\endcsname{1.00}
\expandafter\def\csname v@cnn.fp16.tflip\endcsname{0.0}
\expandafter\def\csname v@cnn.fp32.acc\endcsname{74.7}
\expandafter\def\csname v@cnn.fp32.actkib\endcsname{48.7}
\expandafter\def\csname v@cnn.fp32.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.fp32.f1n2\endcsname{78.4}
\expandafter\def\csname v@cnn.fp32.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.fp32.f1rem\endcsname{64.9}
\expandafter\def\csname v@cnn.fp32.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.fp32.flip\endcsname{0.0}
\expandafter\def\csname v@cnn.fp32.gbops\endcsname{1.064}
\expandafter\def\csname v@cnn.fp32.kappa\endcsname{0.661}
\expandafter\def\csname v@cnn.fp32.kib\endcsname{216.3}
\expandafter\def\csname v@cnn.fp32.mf1\endcsname{69.9}
\expandafter\def\csname v@cnn.fp32.mf1sd\endcsname{0.26}
\expandafter\def\csname v@cnn.fp32.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.fp32ft.acc\endcsname{74.5}
\expandafter\def\csname v@cnn.fp32ft.actkib\endcsname{48.7}
\expandafter\def\csname v@cnn.fp32ft.d\endcsname{\pls{}0.24}
\expandafter\def\csname v@cnn.fp32ft.dabs\endcsname{0.24}
\expandafter\def\csname v@cnn.fp32ft.dhi\endcsname{\pls{}0.56}
\expandafter\def\csname v@cnn.fp32ft.dlo\endcsname{\mns{}0.07}
\expandafter\def\csname v@cnn.fp32ft.f1n1\endcsname{40.4}
\expandafter\def\csname v@cnn.fp32ft.f1n2\endcsname{77.7}
\expandafter\def\csname v@cnn.fp32ft.f1n3\endcsname{76.6}
\expandafter\def\csname v@cnn.fp32ft.f1rem\endcsname{65.6}
\expandafter\def\csname v@cnn.fp32ft.f1w\endcsname{89.6}
\expandafter\def\csname v@cnn.fp32ft.flip\endcsname{7.9}
\expandafter\def\csname v@cnn.fp32ft.gbops\endcsname{1.064}
\expandafter\def\csname v@cnn.fp32ft.kappa\endcsname{0.661}
\expandafter\def\csname v@cnn.fp32ft.kib\endcsname{216.3}
\expandafter\def\csname v@cnn.fp32ft.ltfive\endcsname{0.4}
\expandafter\def\csname v@cnn.fp32ft.lttwo\endcsname{11.1}
\expandafter\def\csname v@cnn.fp32ft.med\endcsname{\pls{}0.23}
\expandafter\def\csname v@cnn.fp32ft.mf1\endcsname{70.0}
\expandafter\def\csname v@cnn.fp32ft.mf1sd\endcsname{0.15}
\expandafter\def\csname v@cnn.fp32ft.n\endcsname{234}
\expandafter\def\csname v@cnn.fp32ft.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.fp32ft.p\endcsname{0.21}
\expandafter\def\csname v@cnn.fp32ft.pfive\endcsname{\mns{}2.98}
\expandafter\def\csname v@cnn.fp32ft.ph\endcsname{0.85}
\expandafter\def\csname v@cnn.fp32ft.tflip\endcsname{7.9}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.acc\endcsname{74.5}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.d\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.dabs\endcsname{0.13}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.dhi\endcsname{\mns{}0.05}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.dlo\endcsname{\mns{}0.22}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.f1n2\endcsname{78.3}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.f1rem\endcsname{64.5}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.f1w\endcsname{89.4}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.flip\endcsname{2.1}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.gbops\endcsname{0.067}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.kappa\endcsname{0.659}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.kib\endcsname{55.3}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.lttwo\endcsname{0.9}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.med\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.mf1\endcsname{69.8}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.mf1sd\endcsname{0.26}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.n\endcsname{234}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.p\endcsname{0.004}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.pfive\endcsname{\mns{}1.11}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.ph\endcsname{0.03}
\expandafter\def\csname v@cnn.fp8e4m3w8a8.tflip\endcsname{2.1}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.acc\endcsname{74.1}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.d\endcsname{\mns{}0.45}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.dabs\endcsname{0.45}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.dhi\endcsname{\mns{}0.22}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.dlo\endcsname{\mns{}0.68}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.f1n1\endcsname{39.8}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.f1n2\endcsname{77.7}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.f1n3\endcsname{77.3}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.f1rem\endcsname{64.1}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.f1w\endcsname{89.3}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.flip\endcsname{4.5}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.gbops\endcsname{0.067}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.kappa\endcsname{0.655}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.kib\endcsname{55.3}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.ltfive\endcsname{0.9}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.lttwo\endcsname{12.0}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.med\endcsname{\mns{}0.32}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.mf1\endcsname{69.7}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.mf1sd\endcsname{0.16}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.n\endcsname{234}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.pfive\endcsname{\mns{}2.95}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.ph\endcsname{0.005}
\expandafter\def\csname v@cnn.fp8e5m2w8a8.tflip\endcsname{4.5}
\expandafter\def\csname v@cnn.fullbudget\endcsname{0}
\expandafter\def\csname v@cnn.int4g32w4.acc\endcsname{74.1}
\expandafter\def\csname v@cnn.int4g32w4.actkib\endcsname{24.3}
\expandafter\def\csname v@cnn.int4g32w4.compr\endcsname{6.1}
\expandafter\def\csname v@cnn.int4g32w4.d\endcsname{\mns{}0.61}
\expandafter\def\csname v@cnn.int4g32w4.dabs\endcsname{0.61}
\expandafter\def\csname v@cnn.int4g32w4.dhi\endcsname{\mns{}0.36}
\expandafter\def\csname v@cnn.int4g32w4.dlo\endcsname{\mns{}0.88}
\expandafter\def\csname v@cnn.int4g32w4.f1n1\endcsname{39.7}
\expandafter\def\csname v@cnn.int4g32w4.f1n2\endcsname{77.7}
\expandafter\def\csname v@cnn.int4g32w4.f1n3\endcsname{76.8}
\expandafter\def\csname v@cnn.int4g32w4.f1rem\endcsname{64.2}
\expandafter\def\csname v@cnn.int4g32w4.f1w\endcsname{89.1}
\expandafter\def\csname v@cnn.int4g32w4.flip\endcsname{5.0}
\expandafter\def\csname v@cnn.int4g32w4.gbops\endcsname{0.067}
\expandafter\def\csname v@cnn.int4g32w4.kappa\endcsname{0.654}
\expandafter\def\csname v@cnn.int4g32w4.kib\endcsname{35.7}
\expandafter\def\csname v@cnn.int4g32w4.ltfive\endcsname{2.6}
\expandafter\def\csname v@cnn.int4g32w4.lttwo\endcsname{12.8}
\expandafter\def\csname v@cnn.int4g32w4.med\endcsname{\mns{}0.56}
\expandafter\def\csname v@cnn.int4g32w4.mf1\endcsname{69.5}
\expandafter\def\csname v@cnn.int4g32w4.mf1sd\endcsname{0.18}
\expandafter\def\csname v@cnn.int4g32w4.n\endcsname{234}
\expandafter\def\csname v@cnn.int4g32w4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.int4g32w4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.int4g32w4.pfive\endcsname{\mns{}3.19}
\expandafter\def\csname v@cnn.int4g32w4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.int4g32w4.tflip\endcsname{5.0}
\expandafter\def\csname v@cnn.int8w8.acc\endcsname{74.7}
\expandafter\def\csname v@cnn.int8w8.actkib\endcsname{48.7}
\expandafter\def\csname v@cnn.int8w8.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@cnn.int8w8.dabs\endcsname{0.02}
\expandafter\def\csname v@cnn.int8w8.dhi\endcsname{\pls{}0.05}
\expandafter\def\csname v@cnn.int8w8.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@cnn.int8w8.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.int8w8.f1n2\endcsname{78.5}
\expandafter\def\csname v@cnn.int8w8.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.int8w8.f1rem\endcsname{64.8}
\expandafter\def\csname v@cnn.int8w8.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.int8w8.flip\endcsname{0.4}
\expandafter\def\csname v@cnn.int8w8.gbops\endcsname{0.266}
\expandafter\def\csname v@cnn.int8w8.kappa\endcsname{0.662}
\expandafter\def\csname v@cnn.int8w8.kib\endcsname{55.3}
\expandafter\def\csname v@cnn.int8w8.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.int8w8.lttwo\endcsname{0.0}
\expandafter\def\csname v@cnn.int8w8.med\endcsname{\pls{}0.01}
\expandafter\def\csname v@cnn.int8w8.mf1\endcsname{69.9}
\expandafter\def\csname v@cnn.int8w8.mf1sd\endcsname{0.24}
\expandafter\def\csname v@cnn.int8w8.n\endcsname{234}
\expandafter\def\csname v@cnn.int8w8.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.int8w8.p\endcsname{0.41}
\expandafter\def\csname v@cnn.int8w8.pfive\endcsname{\mns{}0.33}
\expandafter\def\csname v@cnn.int8w8.ph\endcsname{1.00}
\expandafter\def\csname v@cnn.int8w8.tflip\endcsname{0.4}
\expandafter\def\csname v@cnn.int8w8a8.acc\endcsname{74.6}
\expandafter\def\csname v@cnn.int8w8a8.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.int8w8a8.compr\endcsname{3.9}
\expandafter\def\csname v@cnn.int8w8a8.d\endcsname{\mns{}0.07}
\expandafter\def\csname v@cnn.int8w8a8.dabs\endcsname{0.07}
\expandafter\def\csname v@cnn.int8w8a8.dhi\endcsname{\mns{}0.01}
\expandafter\def\csname v@cnn.int8w8a8.dlo\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.int8w8a8.f1n1\endcsname{39.9}
\expandafter\def\csname v@cnn.int8w8a8.f1n2\endcsname{78.3}
\expandafter\def\csname v@cnn.int8w8a8.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.int8w8a8.f1rem\endcsname{64.6}
\expandafter\def\csname v@cnn.int8w8a8.f1w\endcsname{89.6}
\expandafter\def\csname v@cnn.int8w8a8.flip\endcsname{2.2}
\expandafter\def\csname v@cnn.int8w8a8.gbops\endcsname{0.067}
\expandafter\def\csname v@cnn.int8w8a8.kappa\endcsname{0.660}
\expandafter\def\csname v@cnn.int8w8a8.kib\endcsname{55.3}
\expandafter\def\csname v@cnn.int8w8a8.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.int8w8a8.lttwo\endcsname{0.4}
\expandafter\def\csname v@cnn.int8w8a8.med\endcsname{\mns{}0.05}
\expandafter\def\csname v@cnn.int8w8a8.mf1\endcsname{69.8}
\expandafter\def\csname v@cnn.int8w8a8.mf1sd\endcsname{0.21}
\expandafter\def\csname v@cnn.int8w8a8.n\endcsname{234}
\expandafter\def\csname v@cnn.int8w8a8.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.int8w8a8.p\endcsname{0.04}
\expandafter\def\csname v@cnn.int8w8a8.pfive\endcsname{\mns{}0.76}
\expandafter\def\csname v@cnn.int8w8a8.ph\endcsname{0.30}
\expandafter\def\csname v@cnn.int8w8a8.tflip\endcsname{2.2}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv1.d\endcsname{\mns{}2.35}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv1.dhi\endcsname{\mns{}1.64}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv1.dlo\endcsname{\mns{}3.06}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv1.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv2.d\endcsname{\mns{}0.18}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv2.dhi\endcsname{\mns{}0.07}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv2.dlo\endcsname{\mns{}0.29}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.conv2.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc1.d\endcsname{\mns{}0.11}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc1.dhi\endcsname{\mns{}0.02}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc1.dlo\endcsname{\mns{}0.19}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc1.ph\endcsname{0.004}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc2.d\endcsname{\mns{}0.24}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc2.dhi\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc2.dlo\endcsname{\mns{}0.33}
\expandafter\def\csname v@cnn.ls.mxfp432w4a4.fc2.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv1.d\endcsname{\mns{}1.71}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv1.dhi\endcsname{\mns{}1.17}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv1.dlo\endcsname{\mns{}2.28}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv1.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv2.d\endcsname{\mns{}0.09}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv2.dhi\endcsname{\mns{}0.01}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv2.dlo\endcsname{\mns{}0.17}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.conv2.ph\endcsname{0.06}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc1.d\endcsname{\mns{}0.05}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc1.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc1.dlo\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc1.ph\endcsname{0.03}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc2.d\endcsname{\mns{}0.14}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc2.dhi\endcsname{\mns{}0.07}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc2.dlo\endcsname{\mns{}0.21}
\expandafter\def\csname v@cnn.ls.nvfp416w4a4.fc2.ph\endcsname{0.003}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.acc\endcsname{72.2}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.d\endcsname{\mns{}2.35}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.dabs\endcsname{2.35}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.dhi\endcsname{\mns{}1.64}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.dlo\endcsname{\mns{}3.06}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.f1n1\endcsname{39.3}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.f1n2\endcsname{74.9}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.f1n3\endcsname{78.1}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.f1rem\endcsname{61.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.f1w\endcsname{88.8}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.flip\endcsname{10.7}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.kappa\endcsname{0.630}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.mf1\endcsname{68.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.mf1sd\endcsname{0.25}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv1.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.acc\endcsname{74.4}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.d\endcsname{\mns{}0.18}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.dabs\endcsname{0.18}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.dhi\endcsname{\mns{}0.07}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.dlo\endcsname{\mns{}0.29}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.f1n1\endcsname{39.8}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.f1n2\endcsname{78.3}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.f1n3\endcsname{76.6}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.f1rem\endcsname{64.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.f1w\endcsname{89.4}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.flip\endcsname{3.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.kappa\endcsname{0.659}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.mf1\endcsname{69.7}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.mf1sd\endcsname{0.18}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsmxfp432w4a4conv2.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.acc\endcsname{74.6}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.d\endcsname{\mns{}0.11}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.dabs\endcsname{0.11}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.dhi\endcsname{\mns{}0.02}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.dlo\endcsname{\mns{}0.19}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.f1n1\endcsname{39.8}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.f1n2\endcsname{78.4}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.f1n3\endcsname{76.8}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.f1rem\endcsname{64.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.f1w\endcsname{89.4}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.flip\endcsname{2.7}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.kappa\endcsname{0.660}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.mf1\endcsname{69.8}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.mf1sd\endcsname{0.22}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.p\endcsname{0.001}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc1.ph\endcsname{0.004}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.acc\endcsname{74.4}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.d\endcsname{\mns{}0.24}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.dabs\endcsname{0.24}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.dhi\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.dlo\endcsname{\mns{}0.33}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.f1n1\endcsname{39.9}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.f1n2\endcsname{78.1}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.f1n3\endcsname{76.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.f1rem\endcsname{64.5}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.f1w\endcsname{89.4}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.flip\endcsname{3.0}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.kappa\endcsname{0.658}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.mf1\endcsname{69.7}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.mf1sd\endcsname{0.31}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsmxfp432w4a4fc2.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.acc\endcsname{72.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.d\endcsname{\mns{}1.71}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.dabs\endcsname{1.71}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.dhi\endcsname{\mns{}1.17}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.dlo\endcsname{\mns{}2.28}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.f1n1\endcsname{39.7}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.f1n2\endcsname{75.4}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.f1n3\endcsname{77.4}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.f1rem\endcsname{62.3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.f1w\endcsname{89.3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.flip\endcsname{8.7}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.kappa\endcsname{0.639}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.mf1\endcsname{68.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.mf1sd\endcsname{0.29}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv1.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.acc\endcsname{74.6}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.d\endcsname{\mns{}0.09}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.dabs\endcsname{0.09}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.dhi\endcsname{\mns{}0.01}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.dlo\endcsname{\mns{}0.17}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.f1n1\endcsname{39.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.f1n2\endcsname{78.5}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.f1rem\endcsname{64.6}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.flip\endcsname{2.7}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.kappa\endcsname{0.661}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.mf1\endcsname{69.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.mf1sd\endcsname{0.25}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.p\endcsname{0.06}
\expandafter\def\csname v@cnn.lsnvfp416w4a4conv2.ph\endcsname{0.06}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.acc\endcsname{74.6}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.d\endcsname{\mns{}0.05}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.dabs\endcsname{0.05}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.dlo\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.f1n1\endcsname{39.9}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.f1n2\endcsname{78.4}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.f1n3\endcsname{76.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.f1rem\endcsname{64.6}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.flip\endcsname{2.1}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.kappa\endcsname{0.661}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.mf1\endcsname{69.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.mf1sd\endcsname{0.25}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.p\endcsname{0.01}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc1.ph\endcsname{0.03}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.acc\endcsname{74.5}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.actkib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.d\endcsname{\mns{}0.14}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.dabs\endcsname{0.14}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.dhi\endcsname{\mns{}0.07}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.dlo\endcsname{\mns{}0.21}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.f1n1\endcsname{39.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.f1n2\endcsname{78.3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.f1n3\endcsname{76.3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.f1rem\endcsname{64.8}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.flip\endcsname{2.5}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.gbops\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.kappa\endcsname{0.660}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.kib\endcsname{nan}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.mf1\endcsname{69.7}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.mf1sd\endcsname{0.17}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.lsnvfp416w4a4fc2.ph\endcsname{0.003}
\expandafter\def\csname v@cnn.macs\endcsname{1.04}
\expandafter\def\csname v@cnn.mxfp416w4a4.acc\endcsname{71.5}
\expandafter\def\csname v@cnn.mxfp416w4a4.actkib\endcsname{6.1}
\expandafter\def\csname v@cnn.mxfp416w4a4.d\endcsname{\mns{}3.02}
\expandafter\def\csname v@cnn.mxfp416w4a4.dabs\endcsname{3.02}
\expandafter\def\csname v@cnn.mxfp416w4a4.dhi\endcsname{\mns{}2.26}
\expandafter\def\csname v@cnn.mxfp416w4a4.dlo\endcsname{\mns{}3.77}
\expandafter\def\csname v@cnn.mxfp416w4a4.f1n1\endcsname{38.8}
\expandafter\def\csname v@cnn.mxfp416w4a4.f1n2\endcsname{74.5}
\expandafter\def\csname v@cnn.mxfp416w4a4.f1n3\endcsname{77.5}
\expandafter\def\csname v@cnn.mxfp416w4a4.f1rem\endcsname{60.6}
\expandafter\def\csname v@cnn.mxfp416w4a4.f1w\endcsname{88.5}
\expandafter\def\csname v@cnn.mxfp416w4a4.flip\endcsname{12.5}
\expandafter\def\csname v@cnn.mxfp416w4a4.gbops\endcsname{0.017}
\expandafter\def\csname v@cnn.mxfp416w4a4.kappa\endcsname{0.622}
\expandafter\def\csname v@cnn.mxfp416w4a4.kib\endcsname{31.2}
\expandafter\def\csname v@cnn.mxfp416w4a4.ltfive\endcsname{26.1}
\expandafter\def\csname v@cnn.mxfp416w4a4.lttwo\endcsname{52.6}
\expandafter\def\csname v@cnn.mxfp416w4a4.med\endcsname{\mns{}2.37}
\expandafter\def\csname v@cnn.mxfp416w4a4.mf1\endcsname{68.0}
\expandafter\def\csname v@cnn.mxfp416w4a4.mf1sd\endcsname{0.13}
\expandafter\def\csname v@cnn.mxfp416w4a4.n\endcsname{234}
\expandafter\def\csname v@cnn.mxfp416w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.mxfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp416w4a4.pfive\endcsname{\mns{}10.35}
\expandafter\def\csname v@cnn.mxfp416w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp416w4a4.tflip\endcsname{12.5}
\expandafter\def\csname v@cnn.mxfp432w4.acc\endcsname{73.4}
\expandafter\def\csname v@cnn.mxfp432w4.actkib\endcsname{48.7}
\expandafter\def\csname v@cnn.mxfp432w4.d\endcsname{\mns{}1.30}
\expandafter\def\csname v@cnn.mxfp432w4.dabs\endcsname{1.30}
\expandafter\def\csname v@cnn.mxfp432w4.dhi\endcsname{\mns{}0.90}
\expandafter\def\csname v@cnn.mxfp432w4.dlo\endcsname{\mns{}1.66}
\expandafter\def\csname v@cnn.mxfp432w4.f1n1\endcsname{39.5}
\expandafter\def\csname v@cnn.mxfp432w4.f1n2\endcsname{76.8}
\expandafter\def\csname v@cnn.mxfp432w4.f1n3\endcsname{77.6}
\expandafter\def\csname v@cnn.mxfp432w4.f1rem\endcsname{62.6}
\expandafter\def\csname v@cnn.mxfp432w4.f1w\endcsname{89.0}
\expandafter\def\csname v@cnn.mxfp432w4.flip\endcsname{8.2}
\expandafter\def\csname v@cnn.mxfp432w4.gbops\endcsname{0.133}
\expandafter\def\csname v@cnn.mxfp432w4.kappa\endcsname{0.645}
\expandafter\def\csname v@cnn.mxfp432w4.kib\endcsname{29.7}
\expandafter\def\csname v@cnn.mxfp432w4.ltfive\endcsname{7.3}
\expandafter\def\csname v@cnn.mxfp432w4.lttwo\endcsname{29.9}
\expandafter\def\csname v@cnn.mxfp432w4.med\endcsname{\mns{}0.86}
\expandafter\def\csname v@cnn.mxfp432w4.mf1\endcsname{69.1}
\expandafter\def\csname v@cnn.mxfp432w4.mf1sd\endcsname{0.33}
\expandafter\def\csname v@cnn.mxfp432w4.n\endcsname{234}
\expandafter\def\csname v@cnn.mxfp432w4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.mxfp432w4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4.pfive\endcsname{\mns{}6.23}
\expandafter\def\csname v@cnn.mxfp432w4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4.tflip\endcsname{8.2}
\expandafter\def\csname v@cnn.mxfp432w4a4.acc\endcsname{71.5}
\expandafter\def\csname v@cnn.mxfp432w4a4.actkib\endcsname{6.1}
\expandafter\def\csname v@cnn.mxfp432w4a4.bopsvsfp\endcsname{27}
\expandafter\def\csname v@cnn.mxfp432w4a4.bopsx\endcsname{2.4}
\expandafter\def\csname v@cnn.mxfp432w4a4.compr\endcsname{7.3}
\expandafter\def\csname v@cnn.mxfp432w4a4.d\endcsname{\mns{}3.04}
\expandafter\def\csname v@cnn.mxfp432w4a4.dabs\endcsname{3.04}
\expandafter\def\csname v@cnn.mxfp432w4a4.dhi\endcsname{\mns{}2.31}
\expandafter\def\csname v@cnn.mxfp432w4a4.dlo\endcsname{\mns{}3.77}
\expandafter\def\csname v@cnn.mxfp432w4a4.f1n1\endcsname{38.8}
\expandafter\def\csname v@cnn.mxfp432w4a4.f1n2\endcsname{74.2}
\expandafter\def\csname v@cnn.mxfp432w4a4.f1n3\endcsname{77.5}
\expandafter\def\csname v@cnn.mxfp432w4a4.f1rem\endcsname{60.6}
\expandafter\def\csname v@cnn.mxfp432w4a4.f1w\endcsname{88.5}
\expandafter\def\csname v@cnn.mxfp432w4a4.flip\endcsname{12.6}
\expandafter\def\csname v@cnn.mxfp432w4a4.gbops\endcsname{0.017}
\expandafter\def\csname v@cnn.mxfp432w4a4.kappa\endcsname{0.622}
\expandafter\def\csname v@cnn.mxfp432w4a4.kib\endcsname{29.7}
\expandafter\def\csname v@cnn.mxfp432w4a4.ltfive\endcsname{27.4}
\expandafter\def\csname v@cnn.mxfp432w4a4.lttwo\endcsname{51.3}
\expandafter\def\csname v@cnn.mxfp432w4a4.med\endcsname{\mns{}2.19}
\expandafter\def\csname v@cnn.mxfp432w4a4.mf1\endcsname{67.9}
\expandafter\def\csname v@cnn.mxfp432w4a4.mf1sd\endcsname{0.32}
\expandafter\def\csname v@cnn.mxfp432w4a4.n\endcsname{234}
\expandafter\def\csname v@cnn.mxfp432w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.mxfp432w4a4.ovh\endcsname{2.1}
\expandafter\def\csname v@cnn.mxfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4.pfive\endcsname{\mns{}10.62}
\expandafter\def\csname v@cnn.mxfp432w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4.tflip\endcsname{12.6}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.acc\endcsname{73.9}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.d\endcsname{\mns{}0.69}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.dabs\endcsname{0.69}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.dhi\endcsname{\mns{}0.51}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.dlo\endcsname{\mns{}0.88}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.f1n1\endcsname{39.5}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.f1n2\endcsname{77.8}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.f1rem\endcsname{63.7}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.f1w\endcsname{89.0}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.flip\endcsname{5.7}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.gbops\endcsname{0.039}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.kappa\endcsname{0.652}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.kib\endcsname{30.0}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.lttwo\endcsname{12.4}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.med\endcsname{\mns{}0.51}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.mf1\endcsname{69.4}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.mf1sd\endcsname{0.17}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.n\endcsname{234}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.pfive\endcsname{\mns{}3.00}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8first.tflip\endcsname{5.7}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.acc\endcsname{74.2}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.48}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.dabs\endcsname{0.48}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.dhi\endcsname{\mns{}0.34}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.dlo\endcsname{\mns{}0.61}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.f1n1\endcsname{39.7}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.f1n2\endcsname{78.2}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.f1n3\endcsname{76.7}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.f1rem\endcsname{64.0}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.f1w\endcsname{89.2}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.flip\endcsname{4.8}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.gbops\endcsname{0.039}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.kappa\endcsname{0.656}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.kib\endcsname{30.4}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.lttwo\endcsname{6.0}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.41}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.mf1\endcsname{69.5}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.mf1sd\endcsname{0.08}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.n\endcsname{234}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.pfive\endcsname{\mns{}2.07}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4fp8firstlast.tflip\endcsname{4.8}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.acc\endcsname{73.9}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.actkib\endcsname{6.1}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.ctl\endcsname{\mns{}0.51}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.ctlhi\endcsname{\mns{}0.32}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.ctllo\endcsname{\mns{}0.70}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.ctlph\endcsname{<0.001}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.d\endcsname{\mns{}0.27}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.dabs\endcsname{0.27}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.dhi\endcsname{\pls{}0.04}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.dlo\endcsname{\mns{}0.58}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.f1n2\endcsname{77.0}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.f1n3\endcsname{75.9}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.f1rem\endcsname{64.4}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.f1w\endcsname{89.6}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.flip\endcsname{10.0}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.gbops\endcsname{0.017}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.kappa\endcsname{0.654}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.kib\endcsname{29.7}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.ltfive\endcsname{1.7}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.lttwo\endcsname{18.4}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.med\endcsname{\mns{}0.26}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.mf1\endcsname{69.4}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.mf1sd\endcsname{0.22}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.n\endcsname{234}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.p\endcsname{0.05}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.pfive\endcsname{\mns{}3.91}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.ph\endcsname{0.30}
\expandafter\def\csname v@cnn.mxfp432w4a4qat.tflip\endcsname{10.0}
\expandafter\def\csname v@cnn.noise.ltfive\endcsname{3.0}
\expandafter\def\csname v@cnn.noise.lttwo\endcsname{20.3}
\expandafter\def\csname v@cnn.noise.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@cnn.noise.n\endcsname{468}
\expandafter\def\csname v@cnn.noise.pfive\endcsname{\mns{}4.24}
\expandafter\def\csname v@cnn.noise.tflip\endcsname{15.2}
\expandafter\def\csname v@cnn.nruns\endcsname{30}
\expandafter\def\csname v@cnn.nvfp416w4.acc\endcsname{74.0}
\expandafter\def\csname v@cnn.nvfp416w4.actkib\endcsname{48.7}
\expandafter\def\csname v@cnn.nvfp416w4.d\endcsname{\mns{}0.67}
\expandafter\def\csname v@cnn.nvfp416w4.dabs\endcsname{0.67}
\expandafter\def\csname v@cnn.nvfp416w4.dhi\endcsname{\mns{}0.36}
\expandafter\def\csname v@cnn.nvfp416w4.dlo\endcsname{\mns{}0.98}
\expandafter\def\csname v@cnn.nvfp416w4.f1n1\endcsname{39.8}
\expandafter\def\csname v@cnn.nvfp416w4.f1n2\endcsname{77.5}
\expandafter\def\csname v@cnn.nvfp416w4.f1n3\endcsname{77.0}
\expandafter\def\csname v@cnn.nvfp416w4.f1rem\endcsname{63.6}
\expandafter\def\csname v@cnn.nvfp416w4.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.nvfp416w4.flip\endcsname{6.2}
\expandafter\def\csname v@cnn.nvfp416w4.gbops\endcsname{0.133}
\expandafter\def\csname v@cnn.nvfp416w4.kappa\endcsname{0.653}
\expandafter\def\csname v@cnn.nvfp416w4.kib\endcsname{31.2}
\expandafter\def\csname v@cnn.nvfp416w4.ltfive\endcsname{2.1}
\expandafter\def\csname v@cnn.nvfp416w4.lttwo\endcsname{16.7}
\expandafter\def\csname v@cnn.nvfp416w4.med\endcsname{\mns{}0.54}
\expandafter\def\csname v@cnn.nvfp416w4.mf1\endcsname{69.5}
\expandafter\def\csname v@cnn.nvfp416w4.mf1sd\endcsname{0.27}
\expandafter\def\csname v@cnn.nvfp416w4.n\endcsname{234}
\expandafter\def\csname v@cnn.nvfp416w4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.nvfp416w4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4.pfive\endcsname{\mns{}4.03}
\expandafter\def\csname v@cnn.nvfp416w4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4.tflip\endcsname{6.2}
\expandafter\def\csname v@cnn.nvfp416w4a4.acc\endcsname{72.6}
\expandafter\def\csname v@cnn.nvfp416w4a4.actkib\endcsname{6.1}
\expandafter\def\csname v@cnn.nvfp416w4a4.bopsvsfp\endcsname{27}
\expandafter\def\csname v@cnn.nvfp416w4a4.bopsx\endcsname{2.4}
\expandafter\def\csname v@cnn.nvfp416w4a4.compr\endcsname{6.9}
\expandafter\def\csname v@cnn.nvfp416w4a4.d\endcsname{\mns{}1.98}
\expandafter\def\csname v@cnn.nvfp416w4a4.dabs\endcsname{1.98}
\expandafter\def\csname v@cnn.nvfp416w4a4.dhi\endcsname{\mns{}1.42}
\expandafter\def\csname v@cnn.nvfp416w4a4.dlo\endcsname{\mns{}2.55}
\expandafter\def\csname v@cnn.nvfp416w4a4.f1n1\endcsname{39.4}
\expandafter\def\csname v@cnn.nvfp416w4a4.f1n2\endcsname{75.3}
\expandafter\def\csname v@cnn.nvfp416w4a4.f1n3\endcsname{77.1}
\expandafter\def\csname v@cnn.nvfp416w4a4.f1rem\endcsname{61.9}
\expandafter\def\csname v@cnn.nvfp416w4a4.f1w\endcsname{89.2}
\expandafter\def\csname v@cnn.nvfp416w4a4.flip\endcsname{10.0}
\expandafter\def\csname v@cnn.nvfp416w4a4.gbops\endcsname{0.017}
\expandafter\def\csname v@cnn.nvfp416w4a4.kappa\endcsname{0.636}
\expandafter\def\csname v@cnn.nvfp416w4a4.kib\endcsname{31.2}
\expandafter\def\csname v@cnn.nvfp416w4a4.ltfive\endcsname{15.8}
\expandafter\def\csname v@cnn.nvfp416w4a4.lttwo\endcsname{41.0}
\expandafter\def\csname v@cnn.nvfp416w4a4.med\endcsname{\mns{}1.55}
\expandafter\def\csname v@cnn.nvfp416w4a4.mf1\endcsname{68.6}
\expandafter\def\csname v@cnn.nvfp416w4a4.mf1sd\endcsname{0.23}
\expandafter\def\csname v@cnn.nvfp416w4a4.n\endcsname{234}
\expandafter\def\csname v@cnn.nvfp416w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.nvfp416w4a4.ovh\endcsname{1.8}
\expandafter\def\csname v@cnn.nvfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4a4.pfive\endcsname{\mns{}7.10}
\expandafter\def\csname v@cnn.nvfp416w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4a4.tflip\endcsname{10.0}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.acc\endcsname{74.3}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.d\endcsname{\mns{}0.35}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.dabs\endcsname{0.35}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.dhi\endcsname{\mns{}0.23}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.dlo\endcsname{\mns{}0.47}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.f1n1\endcsname{39.7}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.f1n2\endcsname{78.2}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.f1n3\endcsname{76.6}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.f1rem\endcsname{64.2}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.f1w\endcsname{89.4}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.flip\endcsname{4.6}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.gbops\endcsname{0.039}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.kappa\endcsname{0.657}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.kib\endcsname{31.4}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.lttwo\endcsname{4.3}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.med\endcsname{\mns{}0.44}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.mf1\endcsname{69.6}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.mf1sd\endcsname{0.15}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.n\endcsname{234}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.pfive\endcsname{\mns{}1.84}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8first.tflip\endcsname{4.6}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.acc\endcsname{74.4}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.actkib\endcsname{12.2}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.dabs\endcsname{0.25}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.dhi\endcsname{\mns{}0.13}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.dlo\endcsname{\mns{}0.36}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.f1n1\endcsname{39.9}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.f1n2\endcsname{78.3}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.f1n3\endcsname{76.8}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.f1rem\endcsname{64.3}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.f1w\endcsname{89.5}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.flip\endcsname{3.9}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.gbops\endcsname{0.039}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.kappa\endcsname{0.659}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.kib\endcsname{31.7}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.ltfive\endcsname{0.0}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.lttwo\endcsname{2.6}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.med\endcsname{\mns{}0.24}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.mf1\endcsname{69.7}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.mf1sd\endcsname{0.24}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.n\endcsname{234}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.pfive\endcsname{\mns{}1.55}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.ph\endcsname{0.003}
\expandafter\def\csname v@cnn.nvfp416w4a4fp8firstlast.tflip\endcsname{3.9}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.acc\endcsname{74.0}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.actkib\endcsname{6.1}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.ctl\endcsname{\mns{}0.55}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.ctlhi\endcsname{\mns{}0.37}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.ctllo\endcsname{\mns{}0.73}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.ctlph\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.d\endcsname{\mns{}0.31}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.dabs\endcsname{0.31}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.dhi\endcsname{\pls{}0.05}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.dlo\endcsname{\mns{}0.65}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.f1n1\endcsname{40.0}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.f1n2\endcsname{77.3}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.f1n3\endcsname{76.3}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.f1rem\endcsname{64.6}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.f1w\endcsname{89.3}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.flip\endcsname{9.4}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.gbops\endcsname{0.017}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.kappa\endcsname{0.654}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.kib\endcsname{31.2}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.ltfive\endcsname{3.0}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.lttwo\endcsname{17.1}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.med\endcsname{\mns{}0.14}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.mf1\endcsname{69.5}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.mf1sd\endcsname{0.16}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.n\endcsname{234}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.p\endcsname{0.06}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.pfive\endcsname{\mns{}4.36}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.ph\endcsname{0.30}
\expandafter\def\csname v@cnn.nvfp416w4a4qat.tflip\endcsname{9.4}
\expandafter\def\csname v@cnn.nvfp432w4a4.acc\endcsname{72.2}
\expandafter\def\csname v@cnn.nvfp432w4a4.actkib\endcsname{6.1}
\expandafter\def\csname v@cnn.nvfp432w4a4.d\endcsname{\mns{}2.38}
\expandafter\def\csname v@cnn.nvfp432w4a4.dabs\endcsname{2.38}
\expandafter\def\csname v@cnn.nvfp432w4a4.dhi\endcsname{\mns{}1.76}
\expandafter\def\csname v@cnn.nvfp432w4a4.dlo\endcsname{\mns{}3.04}
\expandafter\def\csname v@cnn.nvfp432w4a4.f1n1\endcsname{39.3}
\expandafter\def\csname v@cnn.nvfp432w4a4.f1n2\endcsname{75.0}
\expandafter\def\csname v@cnn.nvfp432w4a4.f1n3\endcsname{76.9}
\expandafter\def\csname v@cnn.nvfp432w4a4.f1rem\endcsname{61.1}
\expandafter\def\csname v@cnn.nvfp432w4a4.f1w\endcsname{88.8}
\expandafter\def\csname v@cnn.nvfp432w4a4.flip\endcsname{10.9}
\expandafter\def\csname v@cnn.nvfp432w4a4.gbops\endcsname{0.017}
\expandafter\def\csname v@cnn.nvfp432w4a4.kappa\endcsname{0.630}
\expandafter\def\csname v@cnn.nvfp432w4a4.kib\endcsname{29.7}
\expandafter\def\csname v@cnn.nvfp432w4a4.ltfive\endcsname{19.7}
\expandafter\def\csname v@cnn.nvfp432w4a4.lttwo\endcsname{48.3}
\expandafter\def\csname v@cnn.nvfp432w4a4.med\endcsname{\mns{}1.79}
\expandafter\def\csname v@cnn.nvfp432w4a4.mf1\endcsname{68.2}
\expandafter\def\csname v@cnn.nvfp432w4a4.mf1sd\endcsname{0.20}
\expandafter\def\csname v@cnn.nvfp432w4a4.n\endcsname{234}
\expandafter\def\csname v@cnn.nvfp432w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@cnn.nvfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp432w4a4.pfive\endcsname{\mns{}8.39}
\expandafter\def\csname v@cnn.nvfp432w4a4.ph\endcsname{<0.001}
\expandafter\def\csname v@cnn.nvfp432w4a4.tflip\endcsname{10.9}
\expandafter\def\csname v@cnn.params\endcsname{55{,}381}
\expandafter\def\csname v@cnn.valmf\endcsname{70.3}
\expandafter\def\csname v@ctx.bf16.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.bf16.actkib\endcsname{67.4}
\expandafter\def\csname v@ctx.bf16.d\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.bf16.dabs\endcsname{0.01}
\expandafter\def\csname v@ctx.bf16.dhi\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.bf16.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.bf16.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.bf16.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.bf16.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.bf16.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.bf16.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.bf16.flip\endcsname{0.0}
\expandafter\def\csname v@ctx.bf16.gbops\endcsname{1.380}
\expandafter\def\csname v@ctx.bf16.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.bf16.kib\endcsname{746.8}
\expandafter\def\csname v@ctx.bf16.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.bf16.lttwo\endcsname{0.0}
\expandafter\def\csname v@ctx.bf16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.bf16.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.bf16.mf1sd\endcsname{0.80}
\expandafter\def\csname v@ctx.bf16.n\endcsname{234}
\expandafter\def\csname v@ctx.bf16.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.bf16.p\endcsname{0.21}
\expandafter\def\csname v@ctx.bf16.pfive\endcsname{\mns{}0.09}
\expandafter\def\csname v@ctx.bf16.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.bf16.tflip\endcsname{0.0}
\expandafter\def\csname v@ctx.budget\endcsname{40}
\expandafter\def\csname v@ctx.epmed\endcsname{18.5}
\expandafter\def\csname v@ctx.firstmacpct\endcsname{29.2}
\expandafter\def\csname v@ctx.fp16.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.fp16.actkib\endcsname{67.4}
\expandafter\def\csname v@ctx.fp16.compr\endcsname{2.0}
\expandafter\def\csname v@ctx.fp16.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.fp16.dabs\endcsname{0.00}
\expandafter\def\csname v@ctx.fp16.dhi\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.fp16.dlo\endcsname{\mns{}0.00}
\expandafter\def\csname v@ctx.fp16.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.fp16.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.fp16.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.fp16.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.fp16.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.fp16.flip\endcsname{0.0}
\expandafter\def\csname v@ctx.fp16.gbops\endcsname{1.380}
\expandafter\def\csname v@ctx.fp16.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.fp16.kib\endcsname{746.8}
\expandafter\def\csname v@ctx.fp16.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.fp16.lttwo\endcsname{0.0}
\expandafter\def\csname v@ctx.fp16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.fp16.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.fp16.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.fp16.n\endcsname{234}
\expandafter\def\csname v@ctx.fp16.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.fp16.p\endcsname{0.63}
\expandafter\def\csname v@ctx.fp16.pfive\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.fp16.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.fp16.tflip\endcsname{0.0}
\expandafter\def\csname v@ctx.fp32.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.fp32.actkib\endcsname{134.7}
\expandafter\def\csname v@ctx.fp32.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.fp32.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.fp32.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.fp32.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.fp32.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.fp32.flip\endcsname{0.0}
\expandafter\def\csname v@ctx.fp32.gbops\endcsname{5.522}
\expandafter\def\csname v@ctx.fp32.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.fp32.kib\endcsname{1490.3}
\expandafter\def\csname v@ctx.fp32.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.fp32.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.fp32.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.fp32ft.acc\endcsname{80.1}
\expandafter\def\csname v@ctx.fp32ft.actkib\endcsname{134.7}
\expandafter\def\csname v@ctx.fp32ft.d\endcsname{\pls{}0.40}
\expandafter\def\csname v@ctx.fp32ft.dabs\endcsname{0.40}
\expandafter\def\csname v@ctx.fp32ft.dhi\endcsname{\pls{}0.77}
\expandafter\def\csname v@ctx.fp32ft.dlo\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.fp32ft.f1n1\endcsname{50.9}
\expandafter\def\csname v@ctx.fp32ft.f1n2\endcsname{81.9}
\expandafter\def\csname v@ctx.fp32ft.f1n3\endcsname{76.1}
\expandafter\def\csname v@ctx.fp32ft.f1rem\endcsname{79.3}
\expandafter\def\csname v@ctx.fp32ft.f1w\endcsname{91.5}
\expandafter\def\csname v@ctx.fp32ft.flip\endcsname{6.5}
\expandafter\def\csname v@ctx.fp32ft.gbops\endcsname{5.522}
\expandafter\def\csname v@ctx.fp32ft.kappa\endcsname{0.734}
\expandafter\def\csname v@ctx.fp32ft.kib\endcsname{1490.3}
\expandafter\def\csname v@ctx.fp32ft.ltfive\endcsname{2.6}
\expandafter\def\csname v@ctx.fp32ft.lttwo\endcsname{14.5}
\expandafter\def\csname v@ctx.fp32ft.med\endcsname{\pls{}0.35}
\expandafter\def\csname v@ctx.fp32ft.mf1\endcsname{75.9}
\expandafter\def\csname v@ctx.fp32ft.mf1sd\endcsname{0.52}
\expandafter\def\csname v@ctx.fp32ft.n\endcsname{234}
\expandafter\def\csname v@ctx.fp32ft.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.fp32ft.p\endcsname{0.05}
\expandafter\def\csname v@ctx.fp32ft.pfive\endcsname{\mns{}4.01}
\expandafter\def\csname v@ctx.fp32ft.ph\endcsname{0.99}
\expandafter\def\csname v@ctx.fp32ft.tflip\endcsname{6.5}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.dabs\endcsname{0.02}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.dhi\endcsname{\pls{}0.08}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.dlo\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.f1n2\endcsname{81.9}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.f1n3\endcsname{75.7}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.flip\endcsname{0.8}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.gbops\endcsname{0.345}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.kib\endcsname{378.3}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.lttwo\endcsname{0.0}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.med\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.mf1sd\endcsname{0.82}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.n\endcsname{234}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.p\endcsname{0.44}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.pfive\endcsname{\mns{}0.80}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.fp8e4m3w8a8.tflip\endcsname{0.8}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.d\endcsname{\pls{}0.04}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.dabs\endcsname{0.04}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.dhi\endcsname{\pls{}0.18}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.dlo\endcsname{\mns{}0.11}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.f1n1\endcsname{50.2}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.f1n3\endcsname{76.3}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.f1rem\endcsname{78.4}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.f1w\endcsname{91.3}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.flip\endcsname{1.9}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.gbops\endcsname{0.345}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.kib\endcsname{378.3}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.lttwo\endcsname{1.7}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.med\endcsname{\pls{}0.08}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.mf1sd\endcsname{0.78}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.n\endcsname{234}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.p\endcsname{0.33}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.pfive\endcsname{\mns{}1.43}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.fp8e5m2w8a8.tflip\endcsname{1.9}
\expandafter\def\csname v@ctx.fullbudget\endcsname{3}
\expandafter\def\csname v@ctx.int4g32w4.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.int4g32w4.actkib\endcsname{67.4}
\expandafter\def\csname v@ctx.int4g32w4.compr\endcsname{6.2}
\expandafter\def\csname v@ctx.int4g32w4.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.int4g32w4.dabs\endcsname{0.02}
\expandafter\def\csname v@ctx.int4g32w4.dhi\endcsname{\pls{}0.15}
\expandafter\def\csname v@ctx.int4g32w4.dlo\endcsname{\mns{}0.11}
\expandafter\def\csname v@ctx.int4g32w4.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.int4g32w4.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.int4g32w4.f1n3\endcsname{76.0}
\expandafter\def\csname v@ctx.int4g32w4.f1rem\endcsname{78.4}
\expandafter\def\csname v@ctx.int4g32w4.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.int4g32w4.flip\endcsname{1.9}
\expandafter\def\csname v@ctx.int4g32w4.gbops\endcsname{0.345}
\expandafter\def\csname v@ctx.int4g32w4.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.int4g32w4.kib\endcsname{242.0}
\expandafter\def\csname v@ctx.int4g32w4.ltfive\endcsname{0.4}
\expandafter\def\csname v@ctx.int4g32w4.lttwo\endcsname{2.6}
\expandafter\def\csname v@ctx.int4g32w4.med\endcsname{\pls{}0.04}
\expandafter\def\csname v@ctx.int4g32w4.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.int4g32w4.mf1sd\endcsname{0.93}
\expandafter\def\csname v@ctx.int4g32w4.n\endcsname{234}
\expandafter\def\csname v@ctx.int4g32w4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.int4g32w4.p\endcsname{0.55}
\expandafter\def\csname v@ctx.int4g32w4.pfive\endcsname{\mns{}1.42}
\expandafter\def\csname v@ctx.int4g32w4.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.int4g32w4.tflip\endcsname{1.9}
\expandafter\def\csname v@ctx.int8w8.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.int8w8.actkib\endcsname{134.7}
\expandafter\def\csname v@ctx.int8w8.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.int8w8.dabs\endcsname{0.01}
\expandafter\def\csname v@ctx.int8w8.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.int8w8.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.int8w8.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.int8w8.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.int8w8.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.int8w8.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.int8w8.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.int8w8.flip\endcsname{0.1}
\expandafter\def\csname v@ctx.int8w8.gbops\endcsname{1.380}
\expandafter\def\csname v@ctx.int8w8.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.int8w8.kib\endcsname{378.3}
\expandafter\def\csname v@ctx.int8w8.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.int8w8.lttwo\endcsname{0.0}
\expandafter\def\csname v@ctx.int8w8.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.int8w8.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.int8w8.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.int8w8.n\endcsname{234}
\expandafter\def\csname v@ctx.int8w8.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.int8w8.p\endcsname{0.28}
\expandafter\def\csname v@ctx.int8w8.pfive\endcsname{\mns{}0.20}
\expandafter\def\csname v@ctx.int8w8.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.int8w8.tflip\endcsname{0.1}
\expandafter\def\csname v@ctx.int8w8a8.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.int8w8a8.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.int8w8a8.compr\endcsname{3.9}
\expandafter\def\csname v@ctx.int8w8a8.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@ctx.int8w8a8.dabs\endcsname{0.03}
\expandafter\def\csname v@ctx.int8w8a8.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.int8w8a8.dlo\endcsname{\mns{}0.09}
\expandafter\def\csname v@ctx.int8w8a8.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.int8w8a8.f1n2\endcsname{81.8}
\expandafter\def\csname v@ctx.int8w8a8.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.int8w8a8.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.int8w8a8.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.int8w8a8.flip\endcsname{0.7}
\expandafter\def\csname v@ctx.int8w8a8.gbops\endcsname{0.345}
\expandafter\def\csname v@ctx.int8w8a8.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.int8w8a8.kib\endcsname{378.3}
\expandafter\def\csname v@ctx.int8w8a8.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.int8w8a8.lttwo\endcsname{0.0}
\expandafter\def\csname v@ctx.int8w8a8.med\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.int8w8a8.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.int8w8a8.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.int8w8a8.n\endcsname{234}
\expandafter\def\csname v@ctx.int8w8a8.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.int8w8a8.p\endcsname{0.41}
\expandafter\def\csname v@ctx.int8w8a8.pfive\endcsname{\mns{}0.56}
\expandafter\def\csname v@ctx.int8w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.int8w8a8.tflip\endcsname{0.7}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b1conv.d\endcsname{\mns{}0.45}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b1conv.dhi\endcsname{\pls{}0.06}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b1conv.dlo\endcsname{\mns{}1.01}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b1conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b2conv.d\endcsname{\mns{}0.04}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b2conv.dhi\endcsname{\pls{}0.12}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b2conv.dlo\endcsname{\mns{}0.19}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b2conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b3conv.d\endcsname{\pls{}0.05}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b3conv.dhi\endcsname{\pls{}0.19}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b3conv.dlo\endcsname{\mns{}0.07}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.b3conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.cls.d\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.cls.dhi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.cls.dlo\endcsname{\mns{}0.11}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.cls.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.fc.d\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.fc.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.fc.dlo\endcsname{\mns{}0.06}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.fc.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn0.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn0.dhi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn0.dlo\endcsname{\mns{}0.06}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn0.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn1.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn1.dhi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn1.dlo\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn1.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn2.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn2.dhi\endcsname{\mns{}0.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn2.dlo\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn2.ph\endcsname{0.55}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn3.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn3.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn3.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.ls.mxfp432w4a4.tcn3.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b1conv.d\endcsname{\mns{}0.40}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b1conv.dhi\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b1conv.dlo\endcsname{\mns{}0.79}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b1conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b2conv.d\endcsname{\pls{}0.08}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b2conv.dhi\endcsname{\pls{}0.14}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b2conv.dlo\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b2conv.ph\endcsname{0.24}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b3conv.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b3conv.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b3conv.dlo\endcsname{\mns{}0.08}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.b3conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.cls.d\endcsname{\mns{}0.04}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.cls.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.cls.dlo\endcsname{\mns{}0.12}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.cls.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.fc.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.fc.dhi\endcsname{\pls{}0.07}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.fc.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.fc.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn0.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn0.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn0.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn0.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn1.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn1.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn1.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn1.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn2.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn2.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn2.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn2.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn3.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn3.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn3.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.ls.nvfp416w4a4.tcn3.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.acc\endcsname{79.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.d\endcsname{\mns{}0.45}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.dabs\endcsname{0.45}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.dhi\endcsname{\pls{}0.06}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.dlo\endcsname{\mns{}1.01}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.f1n1\endcsname{49.7}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.f1n2\endcsname{81.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.f1n3\endcsname{77.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.f1rem\endcsname{76.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.f1w\endcsname{91.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.flip\endcsname{5.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.kappa\endcsname{0.725}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.mf1sd\endcsname{0.69}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.p\endcsname{0.20}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b1conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.d\endcsname{\mns{}0.04}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.dabs\endcsname{0.04}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.dhi\endcsname{\pls{}0.12}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.dlo\endcsname{\mns{}0.19}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.f1n1\endcsname{50.1}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.f1n2\endcsname{82.2}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.f1n3\endcsname{76.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.f1rem\endcsname{78.2}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.f1w\endcsname{91.1}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.flip\endcsname{1.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.mf1sd\endcsname{0.76}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.p\endcsname{0.97}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b2conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.d\endcsname{\pls{}0.05}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.dabs\endcsname{0.05}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.dhi\endcsname{\pls{}0.19}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.dlo\endcsname{\mns{}0.07}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.f1n1\endcsname{50.2}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.f1n2\endcsname{82.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.f1n3\endcsname{75.7}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.f1rem\endcsname{78.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.f1w\endcsname{91.2}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.flip\endcsname{1.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.mf1\endcsname{75.7}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.mf1sd\endcsname{0.84}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.p\endcsname{0.32}
\expandafter\def\csname v@ctx.lsmxfp432w4a4b3conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.d\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.dabs\endcsname{0.05}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.dhi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.dlo\endcsname{\mns{}0.11}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.f1n2\endcsname{81.8}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.f1n3\endcsname{75.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.f1w\endcsname{91.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.flip\endcsname{1.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.kappa\endcsname{0.730}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.mf1sd\endcsname{0.85}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.p\endcsname{0.07}
\expandafter\def\csname v@ctx.lsmxfp432w4a4cls.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.d\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.dabs\endcsname{0.01}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.dlo\endcsname{\mns{}0.06}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.f1n3\endcsname{75.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.f1w\endcsname{91.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.flip\endcsname{0.7}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.mf1sd\endcsname{0.79}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.p\endcsname{0.23}
\expandafter\def\csname v@ctx.lsmxfp432w4a4fc.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.dabs\endcsname{0.03}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.dhi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.dlo\endcsname{\mns{}0.06}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.f1rem\endcsname{78.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.f1w\endcsname{91.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.flip\endcsname{0.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.mf1sd\endcsname{0.84}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.p\endcsname{0.10}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn0.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.dabs\endcsname{0.02}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.dhi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.dlo\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.flip\endcsname{0.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.p\endcsname{0.10}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn1.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.dabs\endcsname{0.02}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.dhi\endcsname{\mns{}0.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.dlo\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.f1n3\endcsname{75.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.flip\endcsname{0.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.mf1sd\endcsname{0.83}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.p\endcsname{0.03}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn2.ph\endcsname{0.55}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.dabs\endcsname{0.00}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.flip\endcsname{0.4}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.p\endcsname{0.62}
\expandafter\def\csname v@ctx.lsmxfp432w4a4tcn3.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.acc\endcsname{79.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.d\endcsname{\mns{}0.40}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.dabs\endcsname{0.40}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.dhi\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.dlo\endcsname{\mns{}0.79}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.f1n1\endcsname{50.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.f1n2\endcsname{81.2}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.f1n3\endcsname{77.2}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.f1rem\endcsname{77.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.f1w\endcsname{91.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.flip\endcsname{4.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.kappa\endcsname{0.726}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.mf1\endcsname{75.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.mf1sd\endcsname{0.87}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.p\endcsname{0.13}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b1conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.d\endcsname{\pls{}0.08}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.dabs\endcsname{0.08}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.dhi\endcsname{\pls{}0.14}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.dlo\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.f1n2\endcsname{82.1}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.f1n3\endcsname{75.8}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.flip\endcsname{0.8}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.mf1\endcsname{75.7}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.mf1sd\endcsname{0.79}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.p\endcsname{0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b2conv.ph\endcsname{0.24}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.dabs\endcsname{0.03}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.dlo\endcsname{\mns{}0.08}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.f1n1\endcsname{50.2}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.f1rem\endcsname{78.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.f1w\endcsname{91.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.flip\endcsname{0.7}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.mf1sd\endcsname{0.85}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.p\endcsname{0.37}
\expandafter\def\csname v@ctx.lsnvfp416w4a4b3conv.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.d\endcsname{\mns{}0.04}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.dabs\endcsname{0.04}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.dlo\endcsname{\mns{}0.12}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.f1rem\endcsname{78.7}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.f1w\endcsname{91.2}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.flip\endcsname{1.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.kappa\endcsname{0.730}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.mf1sd\endcsname{0.79}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.p\endcsname{0.41}
\expandafter\def\csname v@ctx.lsnvfp416w4a4cls.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.dabs\endcsname{0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.dhi\endcsname{\pls{}0.07}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.f1n2\endcsname{81.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.flip\endcsname{0.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.mf1sd\endcsname{0.80}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.p\endcsname{0.24}
\expandafter\def\csname v@ctx.lsnvfp416w4a4fc.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.dabs\endcsname{0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.flip\endcsname{0.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.mf1sd\endcsname{0.80}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.p\endcsname{0.85}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn0.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.dabs\endcsname{0.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.f1n2\endcsname{81.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.flip\endcsname{0.3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.p\endcsname{0.79}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn1.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.dabs\endcsname{0.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.dlo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.flip\endcsname{0.2}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.p\endcsname{0.86}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn2.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.actkib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.dabs\endcsname{0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.dhi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.dlo\endcsname{\mns{}0.01}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.f1n1\endcsname{50.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.f1n3\endcsname{75.5}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.f1rem\endcsname{78.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.flip\endcsname{0.2}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.gbops\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.kappa\endcsname{0.731}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.kib\endcsname{nan}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.mf1sd\endcsname{0.81}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.p\endcsname{0.69}
\expandafter\def\csname v@ctx.lsnvfp416w4a4tcn3.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.macs\endcsname{5.39}
\expandafter\def\csname v@ctx.mxfp416w4a4.acc\endcsname{79.1}
\expandafter\def\csname v@ctx.mxfp416w4a4.actkib\endcsname{16.8}
\expandafter\def\csname v@ctx.mxfp416w4a4.d\endcsname{\mns{}1.19}
\expandafter\def\csname v@ctx.mxfp416w4a4.dabs\endcsname{1.19}
\expandafter\def\csname v@ctx.mxfp416w4a4.dhi\endcsname{\mns{}0.52}
\expandafter\def\csname v@ctx.mxfp416w4a4.dlo\endcsname{\mns{}1.92}
\expandafter\def\csname v@ctx.mxfp416w4a4.f1n1\endcsname{48.9}
\expandafter\def\csname v@ctx.mxfp416w4a4.f1n2\endcsname{82.1}
\expandafter\def\csname v@ctx.mxfp416w4a4.f1n3\endcsname{78.4}
\expandafter\def\csname v@ctx.mxfp416w4a4.f1rem\endcsname{76.4}
\expandafter\def\csname v@ctx.mxfp416w4a4.f1w\endcsname{90.3}
\expandafter\def\csname v@ctx.mxfp416w4a4.flip\endcsname{7.2}
\expandafter\def\csname v@ctx.mxfp416w4a4.gbops\endcsname{0.086}
\expandafter\def\csname v@ctx.mxfp416w4a4.kappa\endcsname{0.719}
\expandafter\def\csname v@ctx.mxfp416w4a4.kib\endcsname{212.9}
\expandafter\def\csname v@ctx.mxfp416w4a4.ltfive\endcsname{13.7}
\expandafter\def\csname v@ctx.mxfp416w4a4.lttwo\endcsname{32.9}
\expandafter\def\csname v@ctx.mxfp416w4a4.med\endcsname{\mns{}0.67}
\expandafter\def\csname v@ctx.mxfp416w4a4.mf1\endcsname{75.2}
\expandafter\def\csname v@ctx.mxfp416w4a4.mf1sd\endcsname{0.82}
\expandafter\def\csname v@ctx.mxfp416w4a4.n\endcsname{234}
\expandafter\def\csname v@ctx.mxfp416w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.mxfp416w4a4.p\endcsname{0.004}
\expandafter\def\csname v@ctx.mxfp416w4a4.pfive\endcsname{\mns{}8.74}
\expandafter\def\csname v@ctx.mxfp416w4a4.ph\endcsname{0.08}
\expandafter\def\csname v@ctx.mxfp416w4a4.tflip\endcsname{7.2}
\expandafter\def\csname v@ctx.mxfp432w4.acc\endcsname{79.8}
\expandafter\def\csname v@ctx.mxfp432w4.actkib\endcsname{134.7}
\expandafter\def\csname v@ctx.mxfp432w4.d\endcsname{\mns{}0.17}
\expandafter\def\csname v@ctx.mxfp432w4.dabs\endcsname{0.17}
\expandafter\def\csname v@ctx.mxfp432w4.dhi\endcsname{\pls{}0.16}
\expandafter\def\csname v@ctx.mxfp432w4.dlo\endcsname{\mns{}0.53}
\expandafter\def\csname v@ctx.mxfp432w4.f1n1\endcsname{49.9}
\expandafter\def\csname v@ctx.mxfp432w4.f1n2\endcsname{82.2}
\expandafter\def\csname v@ctx.mxfp432w4.f1n3\endcsname{77.1}
\expandafter\def\csname v@ctx.mxfp432w4.f1rem\endcsname{77.7}
\expandafter\def\csname v@ctx.mxfp432w4.f1w\endcsname{91.1}
\expandafter\def\csname v@ctx.mxfp432w4.flip\endcsname{4.0}
\expandafter\def\csname v@ctx.mxfp432w4.gbops\endcsname{0.690}
\expandafter\def\csname v@ctx.mxfp432w4.kappa\endcsname{0.729}
\expandafter\def\csname v@ctx.mxfp432w4.kib\endcsname{201.2}
\expandafter\def\csname v@ctx.mxfp432w4.ltfive\endcsname{3.4}
\expandafter\def\csname v@ctx.mxfp432w4.lttwo\endcsname{12.8}
\expandafter\def\csname v@ctx.mxfp432w4.med\endcsname{\pls{}0.22}
\expandafter\def\csname v@ctx.mxfp432w4.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.mxfp432w4.mf1sd\endcsname{0.74}
\expandafter\def\csname v@ctx.mxfp432w4.n\endcsname{234}
\expandafter\def\csname v@ctx.mxfp432w4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.mxfp432w4.p\endcsname{0.70}
\expandafter\def\csname v@ctx.mxfp432w4.pfive\endcsname{\mns{}3.54}
\expandafter\def\csname v@ctx.mxfp432w4.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.mxfp432w4.tflip\endcsname{4.0}
\expandafter\def\csname v@ctx.mxfp432w4a4.acc\endcsname{79.2}
\expandafter\def\csname v@ctx.mxfp432w4a4.actkib\endcsname{16.8}
\expandafter\def\csname v@ctx.mxfp432w4a4.bopsvsfp\endcsname{34}
\expandafter\def\csname v@ctx.mxfp432w4a4.bopsx\endcsname{1.9}
\expandafter\def\csname v@ctx.mxfp432w4a4.compr\endcsname{7.4}
\expandafter\def\csname v@ctx.mxfp432w4a4.d\endcsname{\mns{}0.91}
\expandafter\def\csname v@ctx.mxfp432w4a4.dabs\endcsname{0.91}
\expandafter\def\csname v@ctx.mxfp432w4a4.dhi\endcsname{\mns{}0.30}
\expandafter\def\csname v@ctx.mxfp432w4a4.dlo\endcsname{\mns{}1.55}
\expandafter\def\csname v@ctx.mxfp432w4a4.f1n1\endcsname{49.1}
\expandafter\def\csname v@ctx.mxfp432w4a4.f1n2\endcsname{82.0}
\expandafter\def\csname v@ctx.mxfp432w4a4.f1n3\endcsname{78.2}
\expandafter\def\csname v@ctx.mxfp432w4a4.f1rem\endcsname{76.7}
\expandafter\def\csname v@ctx.mxfp432w4a4.f1w\endcsname{90.6}
\expandafter\def\csname v@ctx.mxfp432w4a4.flip\endcsname{6.5}
\expandafter\def\csname v@ctx.mxfp432w4a4.gbops\endcsname{0.086}
\expandafter\def\csname v@ctx.mxfp432w4a4.kappa\endcsname{0.722}
\expandafter\def\csname v@ctx.mxfp432w4a4.kib\endcsname{201.2}
\expandafter\def\csname v@ctx.mxfp432w4a4.ltfive\endcsname{11.1}
\expandafter\def\csname v@ctx.mxfp432w4a4.lttwo\endcsname{26.1}
\expandafter\def\csname v@ctx.mxfp432w4a4.med\endcsname{\mns{}0.46}
\expandafter\def\csname v@ctx.mxfp432w4a4.mf1\endcsname{75.3}
\expandafter\def\csname v@ctx.mxfp432w4a4.mf1sd\endcsname{0.66}
\expandafter\def\csname v@ctx.mxfp432w4a4.n\endcsname{234}
\expandafter\def\csname v@ctx.mxfp432w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.mxfp432w4a4.ovh\endcsname{0.8}
\expandafter\def\csname v@ctx.mxfp432w4a4.p\endcsname{0.02}
\expandafter\def\csname v@ctx.mxfp432w4a4.pfive\endcsname{\mns{}7.47}
\expandafter\def\csname v@ctx.mxfp432w4a4.ph\endcsname{0.30}
\expandafter\def\csname v@ctx.mxfp432w4a4.tflip\endcsname{6.5}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.acc\endcsname{79.8}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.d\endcsname{\mns{}0.23}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.dabs\endcsname{0.23}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.dhi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.dlo\endcsname{\mns{}0.53}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.f1n1\endcsname{49.5}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.f1n2\endcsname{82.6}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.f1n3\endcsname{76.9}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.f1rem\endcsname{78.2}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.f1w\endcsname{90.5}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.flip\endcsname{3.6}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.gbops\endcsname{0.162}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.kappa\endcsname{0.729}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.kib\endcsname{202.5}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.ltfive\endcsname{2.6}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.lttwo\endcsname{12.0}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.med\endcsname{\mns{}0.03}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.mf1sd\endcsname{0.91}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.n\endcsname{234}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.p\endcsname{0.41}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.pfive\endcsname{\mns{}3.51}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8first.tflip\endcsname{3.6}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.acc\endcsname{79.8}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.13}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.dabs\endcsname{0.13}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.dhi\endcsname{\pls{}0.11}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.dlo\endcsname{\mns{}0.40}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.f1n1\endcsname{49.6}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.f1n2\endcsname{82.7}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.f1n3\endcsname{77.0}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.f1rem\endcsname{78.2}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.f1w\endcsname{90.5}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.flip\endcsname{3.2}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.gbops\endcsname{0.162}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.kappa\endcsname{0.730}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.kib\endcsname{202.8}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.ltfive\endcsname{2.1}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.lttwo\endcsname{10.7}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.med\endcsname{\pls{}0.04}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.mf1sd\endcsname{0.87}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.n\endcsname{234}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.p\endcsname{0.96}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.pfive\endcsname{\mns{}3.19}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.mxfp432w4a4fp8firstlast.tflip\endcsname{3.2}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.actkib\endcsname{16.8}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.ctl\endcsname{\mns{}0.21}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.ctlhi\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.ctllo\endcsname{\mns{}0.41}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.ctlph\endcsname{0.03}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.d\endcsname{\pls{}0.19}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.dabs\endcsname{0.19}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.dhi\endcsname{\pls{}0.54}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.dlo\endcsname{\mns{}0.18}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.f1n1\endcsname{50.6}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.f1n2\endcsname{81.8}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.f1n3\endcsname{75.8}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.f1rem\endcsname{79.0}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.flip\endcsname{6.8}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.gbops\endcsname{0.086}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.kib\endcsname{201.2}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.ltfive\endcsname{3.8}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.lttwo\endcsname{16.7}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.med\endcsname{\pls{}0.13}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.mf1\endcsname{75.7}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.mf1sd\endcsname{0.84}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.n\endcsname{234}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.p\endcsname{0.53}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.pfive\endcsname{\mns{}3.82}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.mxfp432w4a4qat.tflip\endcsname{6.8}
\expandafter\def\csname v@ctx.noise.ltfive\endcsname{10.7}
\expandafter\def\csname v@ctx.noise.lttwo\endcsname{24.1}
\expandafter\def\csname v@ctx.noise.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.noise.n\endcsname{468}
\expandafter\def\csname v@ctx.noise.pfive\endcsname{\mns{}6.10}
\expandafter\def\csname v@ctx.noise.tflip\endcsname{9.4}
\expandafter\def\csname v@ctx.nruns\endcsname{30}
\expandafter\def\csname v@ctx.nvfp416w4.acc\endcsname{79.7}
\expandafter\def\csname v@ctx.nvfp416w4.actkib\endcsname{134.7}
\expandafter\def\csname v@ctx.nvfp416w4.d\endcsname{\mns{}0.14}
\expandafter\def\csname v@ctx.nvfp416w4.dabs\endcsname{0.14}
\expandafter\def\csname v@ctx.nvfp416w4.dhi\endcsname{\pls{}0.05}
\expandafter\def\csname v@ctx.nvfp416w4.dlo\endcsname{\mns{}0.33}
\expandafter\def\csname v@ctx.nvfp416w4.f1n1\endcsname{50.1}
\expandafter\def\csname v@ctx.nvfp416w4.f1n2\endcsname{81.8}
\expandafter\def\csname v@ctx.nvfp416w4.f1n3\endcsname{76.4}
\expandafter\def\csname v@ctx.nvfp416w4.f1rem\endcsname{78.1}
\expandafter\def\csname v@ctx.nvfp416w4.f1w\endcsname{91.2}
\expandafter\def\csname v@ctx.nvfp416w4.flip\endcsname{3.0}
\expandafter\def\csname v@ctx.nvfp416w4.gbops\endcsname{0.690}
\expandafter\def\csname v@ctx.nvfp416w4.kappa\endcsname{0.728}
\expandafter\def\csname v@ctx.nvfp416w4.kib\endcsname{212.9}
\expandafter\def\csname v@ctx.nvfp416w4.ltfive\endcsname{0.4}
\expandafter\def\csname v@ctx.nvfp416w4.lttwo\endcsname{10.3}
\expandafter\def\csname v@ctx.nvfp416w4.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@ctx.nvfp416w4.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.nvfp416w4.mf1sd\endcsname{0.86}
\expandafter\def\csname v@ctx.nvfp416w4.n\endcsname{234}
\expandafter\def\csname v@ctx.nvfp416w4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.nvfp416w4.p\endcsname{0.26}
\expandafter\def\csname v@ctx.nvfp416w4.pfive\endcsname{\mns{}2.89}
\expandafter\def\csname v@ctx.nvfp416w4.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.nvfp416w4.tflip\endcsname{3.0}
\expandafter\def\csname v@ctx.nvfp416w4a4.acc\endcsname{79.4}
\expandafter\def\csname v@ctx.nvfp416w4a4.actkib\endcsname{16.8}
\expandafter\def\csname v@ctx.nvfp416w4a4.bopsvsfp\endcsname{34}
\expandafter\def\csname v@ctx.nvfp416w4a4.bopsx\endcsname{1.9}
\expandafter\def\csname v@ctx.nvfp416w4a4.compr\endcsname{7.0}
\expandafter\def\csname v@ctx.nvfp416w4a4.d\endcsname{\mns{}0.49}
\expandafter\def\csname v@ctx.nvfp416w4a4.dabs\endcsname{0.49}
\expandafter\def\csname v@ctx.nvfp416w4a4.dhi\endcsname{\mns{}0.05}
\expandafter\def\csname v@ctx.nvfp416w4a4.dlo\endcsname{\mns{}0.93}
\expandafter\def\csname v@ctx.nvfp416w4a4.f1n1\endcsname{49.8}
\expandafter\def\csname v@ctx.nvfp416w4a4.f1n2\endcsname{81.4}
\expandafter\def\csname v@ctx.nvfp416w4a4.f1n3\endcsname{77.4}
\expandafter\def\csname v@ctx.nvfp416w4a4.f1rem\endcsname{77.2}
\expandafter\def\csname v@ctx.nvfp416w4a4.f1w\endcsname{91.3}
\expandafter\def\csname v@ctx.nvfp416w4a4.flip\endcsname{5.2}
\expandafter\def\csname v@ctx.nvfp416w4a4.gbops\endcsname{0.086}
\expandafter\def\csname v@ctx.nvfp416w4a4.kappa\endcsname{0.725}
\expandafter\def\csname v@ctx.nvfp416w4a4.kib\endcsname{212.9}
\expandafter\def\csname v@ctx.nvfp416w4a4.ltfive\endcsname{6.8}
\expandafter\def\csname v@ctx.nvfp416w4a4.lttwo\endcsname{21.4}
\expandafter\def\csname v@ctx.nvfp416w4a4.med\endcsname{\mns{}0.04}
\expandafter\def\csname v@ctx.nvfp416w4a4.mf1\endcsname{75.4}
\expandafter\def\csname v@ctx.nvfp416w4a4.mf1sd\endcsname{0.79}
\expandafter\def\csname v@ctx.nvfp416w4a4.n\endcsname{234}
\expandafter\def\csname v@ctx.nvfp416w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.nvfp416w4a4.ovh\endcsname{0.7}
\expandafter\def\csname v@ctx.nvfp416w4a4.p\endcsname{0.07}
\expandafter\def\csname v@ctx.nvfp416w4a4.pfive\endcsname{\mns{}5.42}
\expandafter\def\csname v@ctx.nvfp416w4a4.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.nvfp416w4a4.tflip\endcsname{5.2}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.acc\endcsname{79.9}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.d\endcsname{\pls{}0.02}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.dabs\endcsname{0.02}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.dhi\endcsname{\pls{}0.15}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.dlo\endcsname{\mns{}0.11}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.f1n1\endcsname{50.2}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.f1n2\endcsname{82.1}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.f1n3\endcsname{76.1}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.f1rem\endcsname{78.5}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.f1w\endcsname{91.1}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.flip\endcsname{2.2}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.gbops\endcsname{0.162}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.kappa\endcsname{0.730}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.kib\endcsname{214.0}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.lttwo\endcsname{2.1}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.med\endcsname{\pls{}0.05}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.mf1sd\endcsname{0.82}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.n\endcsname{234}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.p\endcsname{0.35}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.pfive\endcsname{\mns{}1.51}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8first.tflip\endcsname{2.2}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.acc\endcsname{80.0}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.actkib\endcsname{33.7}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.06}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.dabs\endcsname{0.06}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.dhi\endcsname{\pls{}0.15}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.dlo\endcsname{\mns{}0.04}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.f1n1\endcsname{50.3}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.f1n2\endcsname{82.1}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.f1n3\endcsname{76.0}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.f1rem\endcsname{78.4}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.flip\endcsname{1.6}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.gbops\endcsname{0.162}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.kappa\endcsname{0.732}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.kib\endcsname{214.3}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.ltfive\endcsname{0.0}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.lttwo\endcsname{1.3}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.10}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.mf1\endcsname{75.6}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.mf1sd\endcsname{0.84}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.n\endcsname{234}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.p\endcsname{0.07}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.pfive\endcsname{\mns{}1.32}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.nvfp416w4a4fp8firstlast.tflip\endcsname{1.6}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.acc\endcsname{80.2}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.actkib\endcsname{16.8}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.ctl\endcsname{\pls{}0.03}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.ctlhi\endcsname{\pls{}0.22}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.ctllo\endcsname{\mns{}0.16}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.ctlph\endcsname{0.64}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.d\endcsname{\pls{}0.43}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.dabs\endcsname{0.43}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.dhi\endcsname{\pls{}0.81}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.dlo\endcsname{\pls{}0.04}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.f1n1\endcsname{51.0}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.f1n2\endcsname{82.1}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.f1n3\endcsname{76.0}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.f1rem\endcsname{79.5}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.f1w\endcsname{91.5}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.flip\endcsname{6.6}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.gbops\endcsname{0.086}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.kappa\endcsname{0.735}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.kib\endcsname{212.9}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.ltfive\endcsname{2.6}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.lttwo\endcsname{12.8}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.med\endcsname{\pls{}0.35}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.mf1\endcsname{76.0}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.mf1sd\endcsname{0.41}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.n\endcsname{234}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.p\endcsname{0.06}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.pfive\endcsname{\mns{}4.18}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.ph\endcsname{0.99}
\expandafter\def\csname v@ctx.nvfp416w4a4qat.tflip\endcsname{6.6}
\expandafter\def\csname v@ctx.nvfp432w4a4.acc\endcsname{79.6}
\expandafter\def\csname v@ctx.nvfp432w4a4.actkib\endcsname{16.8}
\expandafter\def\csname v@ctx.nvfp432w4a4.d\endcsname{\mns{}0.39}
\expandafter\def\csname v@ctx.nvfp432w4a4.dabs\endcsname{0.39}
\expandafter\def\csname v@ctx.nvfp432w4a4.dhi\endcsname{\pls{}0.09}
\expandafter\def\csname v@ctx.nvfp432w4a4.dlo\endcsname{\mns{}0.88}
\expandafter\def\csname v@ctx.nvfp432w4a4.f1n1\endcsname{49.9}
\expandafter\def\csname v@ctx.nvfp432w4a4.f1n2\endcsname{81.6}
\expandafter\def\csname v@ctx.nvfp432w4a4.f1n3\endcsname{77.7}
\expandafter\def\csname v@ctx.nvfp432w4a4.f1rem\endcsname{77.0}
\expandafter\def\csname v@ctx.nvfp432w4a4.f1w\endcsname{91.4}
\expandafter\def\csname v@ctx.nvfp432w4a4.flip\endcsname{5.4}
\expandafter\def\csname v@ctx.nvfp432w4a4.gbops\endcsname{0.086}
\expandafter\def\csname v@ctx.nvfp432w4a4.kappa\endcsname{0.726}
\expandafter\def\csname v@ctx.nvfp432w4a4.kib\endcsname{201.2}
\expandafter\def\csname v@ctx.nvfp432w4a4.ltfive\endcsname{6.4}
\expandafter\def\csname v@ctx.nvfp432w4a4.lttwo\endcsname{21.8}
\expandafter\def\csname v@ctx.nvfp432w4a4.med\endcsname{\mns{}0.11}
\expandafter\def\csname v@ctx.nvfp432w4a4.mf1\endcsname{75.5}
\expandafter\def\csname v@ctx.nvfp432w4a4.mf1sd\endcsname{0.67}
\expandafter\def\csname v@ctx.nvfp432w4a4.n\endcsname{234}
\expandafter\def\csname v@ctx.nvfp432w4a4.nseeds\endcsname{3}
\expandafter\def\csname v@ctx.nvfp432w4a4.p\endcsname{0.29}
\expandafter\def\csname v@ctx.nvfp432w4a4.pfive\endcsname{\mns{}5.37}
\expandafter\def\csname v@ctx.nvfp432w4a4.ph\endcsname{1.00}
\expandafter\def\csname v@ctx.nvfp432w4a4.tflip\endcsname{5.4}
\expandafter\def\csname v@ctx.params\endcsname{381{,}701}
\expandafter\def\csname v@ctx.valmf\endcsname{75.9}
\expandafter\def\csname v@data.calib\endcsname{1{,}020}
\expandafter\def\csname v@data.calibper\endcsname{204}
\expandafter\def\csname v@data.nI\endcsname{21{,}522}
\expandafter\def\csname v@data.nII\endcsname{69{,}132}
\expandafter\def\csname v@data.nIII\endcsname{13{,}039}
\expandafter\def\csname v@data.nIIIpct\endcsname{6.7}
\expandafter\def\csname v@data.nIIpct\endcsname{35.4}
\expandafter\def\csname v@data.nIpct\endcsname{11.0}
\expandafter\def\csname v@data.nights\endcsname{153}
\expandafter\def\csname v@data.rem\endcsname{25{,}835}
\expandafter\def\csname v@data.rempct\endcsname{13.2}
\expandafter\def\csname v@data.subjects\endcsname{78}
\expandafter\def\csname v@data.total\endcsname{195{,}469}
\expandafter\def\csname v@data.w\endcsname{65{,}941}
\expandafter\def\csname v@data.wpct\endcsname{33.7}
\expandafter\def\csname v@eightbit.maxabs\endcsname{0.45}
\expandafter\def\csname v@enc.params\endcsname{184{,}581}
\expandafter\def\csname v@flqat.himax\endcsname{\pls{}0.46}
\expandafter\def\csname v@flqat.lomin\endcsname{\mns{}0.85}
\expandafter\def\csname v@flqat.max\endcsname{\pls{}0.06}
\expandafter\def\csname v@flqat.min\endcsname{\mns{}0.37}
\expandafter\def\csname v@flqat.nqat\endcsname{three}
\expandafter\def\csname v@flqat.phmin\endcsname{0.60}
\expandafter\def\csname v@fp32.sd.max\endcsname{0.81}
\expandafter\def\csname v@fp32.sd.min\endcsname{0.26}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.ftptq.d\endcsname{\mns{}2.31}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.ftptq.hi\endcsname{\mns{}1.59}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.ftptq.lo\endcsname{\mns{}3.03}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.ftptq.med\endcsname{\mns{}1.90}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.ftptq.p\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.qatminus.d\endcsname{\pls{}2.04}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.qatminus.hi\endcsname{\pls{}2.76}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.qatminus.lo\endcsname{\pls{}1.34}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.qatminus.med\endcsname{\pls{}1.28}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.qatminus.p\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.qatminus.ph\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.vsft.d\endcsname{\mns{}2.55}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.vsft.hi\endcsname{\mns{}1.83}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.vsft.lo\endcsname{\mns{}3.29}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.vsft.med\endcsname{\mns{}1.94}
\expandafter\def\csname v@ftptq.cnn.mxfp432w4a4.vsft.p\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.ftptq.d\endcsname{\mns{}2.18}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.ftptq.hi\endcsname{\mns{}1.56}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.ftptq.lo\endcsname{\mns{}2.84}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.ftptq.med\endcsname{\mns{}1.67}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.ftptq.p\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.qatminus.d\endcsname{\pls{}1.87}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.qatminus.hi\endcsname{\pls{}2.48}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.qatminus.lo\endcsname{\pls{}1.30}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.qatminus.med\endcsname{\pls{}1.45}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.qatminus.p\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.qatminus.ph\endcsname{<0.001}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.vsft.d\endcsname{\mns{}2.42}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.vsft.hi\endcsname{\mns{}1.82}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.vsft.lo\endcsname{\mns{}3.06}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.vsft.med\endcsname{\mns{}1.93}
\expandafter\def\csname v@ftptq.cnn.nvfp416w4a4.vsft.p\endcsname{<0.001}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.ftptq.d\endcsname{\mns{}0.91}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.ftptq.hi\endcsname{\mns{}0.10}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.ftptq.lo\endcsname{\mns{}1.76}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.ftptq.med\endcsname{\mns{}0.10}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.ftptq.p\endcsname{0.10}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.qatminus.d\endcsname{\pls{}1.09}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.qatminus.hi\endcsname{\pls{}1.94}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.qatminus.lo\endcsname{\pls{}0.31}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.qatminus.med\endcsname{\pls{}0.20}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.qatminus.p\endcsname{0.04}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.qatminus.ph\endcsname{0.08}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.vsft.d\endcsname{\mns{}1.30}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.vsft.hi\endcsname{\mns{}0.54}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.vsft.lo\endcsname{\mns{}2.10}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.vsft.med\endcsname{\mns{}0.85}
\expandafter\def\csname v@ftptq.ctx.mxfp432w4a4.vsft.p\endcsname{0.006}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.ftptq.d\endcsname{\mns{}0.16}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.ftptq.hi\endcsname{\pls{}0.48}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.ftptq.lo\endcsname{\mns{}0.81}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.ftptq.med\endcsname{\pls{}0.05}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.ftptq.p\endcsname{0.85}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.qatminus.d\endcsname{\pls{}0.59}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.qatminus.hi\endcsname{\pls{}1.13}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.qatminus.lo\endcsname{\pls{}0.06}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.qatminus.med\endcsname{\pls{}0.19}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.qatminus.p\endcsname{0.09}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.qatminus.ph\endcsname{0.09}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.vsft.d\endcsname{\mns{}0.56}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.vsft.hi\endcsname{\mns{}0.02}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.vsft.lo\endcsname{\mns{}1.11}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.vsft.med\endcsname{\mns{}0.19}
\expandafter\def\csname v@ftptq.ctx.nvfp416w4a4.vsft.p\endcsname{0.12}
\expandafter\def\csname v@gapaw.diff.fp8e4m3w8a8.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@gapaw.diff.fp8e4m3w8a8.hi\endcsname{\pls{}0.07}
\expandafter\def\csname v@gapaw.diff.fp8e4m3w8a8.lo\endcsname{\mns{}0.12}
\expandafter\def\csname v@gapaw.diff.fp8e4m3w8a8.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@gapaw.diff.fp8e4m3w8a8.p\endcsname{0.96}
\expandafter\def\csname v@gapaw.diff.int8w8a8.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@gapaw.diff.int8w8a8.hi\endcsname{\pls{}0.06}
\expandafter\def\csname v@gapaw.diff.int8w8a8.lo\endcsname{\mns{}0.04}
\expandafter\def\csname v@gapaw.diff.int8w8a8.med\endcsname{\pls{}0.03}
\expandafter\def\csname v@gapaw.diff.int8w8a8.p\endcsname{0.67}
\expandafter\def\csname v@gapaw.diff.maxabs\endcsname{0.23}
\expandafter\def\csname v@gapaw.diff.mxfp416w4a4.d\endcsname{\pls{}0.10}
\expandafter\def\csname v@gapaw.diff.mxfp416w4a4.hi\endcsname{\pls{}0.51}
\expandafter\def\csname v@gapaw.diff.mxfp416w4a4.lo\endcsname{\mns{}0.32}
\expandafter\def\csname v@gapaw.diff.mxfp416w4a4.med\endcsname{\mns{}0.04}
\expandafter\def\csname v@gapaw.diff.mxfp416w4a4.p\endcsname{0.71}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4.d\endcsname{\pls{}0.12}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4.hi\endcsname{\pls{}0.52}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4.lo\endcsname{\mns{}0.26}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4.med\endcsname{\mns{}0.03}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4.p\endcsname{0.81}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.09}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.13}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.29}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.09}
\expandafter\def\csname v@gapaw.diff.mxfp432w4a4fp8firstlast.p\endcsname{0.30}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4.d\endcsname{\pls{}0.23}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4.hi\endcsname{\pls{}0.55}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4.lo\endcsname{\mns{}0.06}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4.med\endcsname{\pls{}0.16}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4.p\endcsname{0.22}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4fp8firstlast.d\endcsname{\mns{}0.09}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.05}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.25}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4fp8firstlast.med\endcsname{\mns{}0.11}
\expandafter\def\csname v@gapaw.diff.nvfp416w4a4fp8firstlast.p\endcsname{0.19}
\expandafter\def\csname v@gapaw.diff.nvfp432w4a4.d\endcsname{\pls{}0.16}
\expandafter\def\csname v@gapaw.diff.nvfp432w4a4.hi\endcsname{\pls{}0.52}
\expandafter\def\csname v@gapaw.diff.nvfp432w4a4.lo\endcsname{\mns{}0.20}
\expandafter\def\csname v@gapaw.diff.nvfp432w4a4.med\endcsname{\pls{}0.11}
\expandafter\def\csname v@gapaw.diff.nvfp432w4a4.p\endcsname{0.69}
\expandafter\def\csname v@gapaw.fp32.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@gapaw.fp32.hi\endcsname{\pls{}0.24}
\expandafter\def\csname v@gapaw.fp32.lo\endcsname{\mns{}0.77}
\expandafter\def\csname v@gapaw.fp32.med\endcsname{\mns{}0.15}
\expandafter\def\csname v@gapaw.fp32.mf1\endcsname{75.3}
\expandafter\def\csname v@gapaw.fp32.p\endcsname{0.55}
\expandafter\def\csname v@gapaw.fp8e4m3w8a8.d\endcsname{\mns{}0.01}
\expandafter\def\csname v@gapaw.fp8e4m3w8a8.hi\endcsname{\pls{}0.05}
\expandafter\def\csname v@gapaw.fp8e4m3w8a8.lo\endcsname{\mns{}0.07}
\expandafter\def\csname v@gapaw.fp8e4m3w8a8.med\endcsname{\pls{}0.04}
\expandafter\def\csname v@gapaw.fp8e4m3w8a8.p\endcsname{0.34}
\expandafter\def\csname v@gapaw.int8w8a8.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@gapaw.int8w8a8.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@gapaw.int8w8a8.lo\endcsname{\mns{}0.06}
\expandafter\def\csname v@gapaw.int8w8a8.med\endcsname{\mns{}0.03}
\expandafter\def\csname v@gapaw.int8w8a8.p\endcsname{0.36}
\expandafter\def\csname v@gapaw.mxfp416w4a4.d\endcsname{\mns{}1.10}
\expandafter\def\csname v@gapaw.mxfp416w4a4.hi\endcsname{\mns{}0.35}
\expandafter\def\csname v@gapaw.mxfp416w4a4.lo\endcsname{\mns{}1.88}
\expandafter\def\csname v@gapaw.mxfp416w4a4.med\endcsname{\mns{}0.92}
\expandafter\def\csname v@gapaw.mxfp416w4a4.p\endcsname{0.02}
\expandafter\def\csname v@gapaw.mxfp432w4a4.d\endcsname{\mns{}0.79}
\expandafter\def\csname v@gapaw.mxfp432w4a4.hi\endcsname{\mns{}0.15}
\expandafter\def\csname v@gapaw.mxfp432w4a4.lo\endcsname{\mns{}1.42}
\expandafter\def\csname v@gapaw.mxfp432w4a4.med\endcsname{\mns{}0.26}
\expandafter\def\csname v@gapaw.mxfp432w4a4.p\endcsname{0.07}
\expandafter\def\csname v@gapaw.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.22}
\expandafter\def\csname v@gapaw.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.03}
\expandafter\def\csname v@gapaw.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.49}
\expandafter\def\csname v@gapaw.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.18}
\expandafter\def\csname v@gapaw.mxfp432w4a4fp8firstlast.p\endcsname{0.26}
\expandafter\def\csname v@gapaw.nvfp416w4a4.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@gapaw.nvfp416w4a4.hi\endcsname{\pls{}0.18}
\expandafter\def\csname v@gapaw.nvfp416w4a4.lo\endcsname{\mns{}0.70}
\expandafter\def\csname v@gapaw.nvfp416w4a4.med\endcsname{\mns{}0.02}
\expandafter\def\csname v@gapaw.nvfp416w4a4.p\endcsname{0.55}
\expandafter\def\csname v@gapaw.nvfp416w4a4fp8firstlast.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@gapaw.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.09}
\expandafter\def\csname v@gapaw.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.16}
\expandafter\def\csname v@gapaw.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.06}
\expandafter\def\csname v@gapaw.nvfp416w4a4fp8firstlast.p\endcsname{0.84}
\expandafter\def\csname v@gapaw.nvfp432w4a4.d\endcsname{\mns{}0.23}
\expandafter\def\csname v@gapaw.nvfp432w4a4.hi\endcsname{\pls{}0.24}
\expandafter\def\csname v@gapaw.nvfp432w4a4.lo\endcsname{\mns{}0.71}
\expandafter\def\csname v@gapaw.nvfp432w4a4.med\endcsname{\pls{}0.04}
\expandafter\def\csname v@gapaw.nvfp432w4a4.p\endcsname{0.80}
\expandafter\def\csname v@gaps.maxlen\endcsname{97}
\expandafter\def\csname v@gaps.medlen\endcsname{1}
\expandafter\def\csname v@gaps.n\endcsname{140}
\expandafter\def\csname v@gaps.near\endcsname{3{,}601}
\expandafter\def\csname v@gaps.nearpct\endcsname{1.84}
\expandafter\def\csname v@gaps.nights\endcsname{153}
\expandafter\def\csname v@gaps.removed\endcsname{288}
\expandafter\def\csname v@gaps.withgap\endcsname{47}
\expandafter\def\csname v@gemm.contextsleepnet.b1conv.bf16\endcsname{14.4}
\expandafter\def\csname v@gemm.contextsleepnet.b1conv.fp32\endcsname{32.8}
\expandafter\def\csname v@gemm.contextsleepnet.b1conv.fp8\endcsname{10.3}
\expandafter\def\csname v@gemm.contextsleepnet.b1conv.mkn\endcsname{125952\times64\times64}
\expandafter\def\csname v@gemm.contextsleepnet.b2conv.bf16\endcsname{8.2}
\expandafter\def\csname v@gemm.contextsleepnet.b2conv.fp32\endcsname{41.0}
\expandafter\def\csname v@gemm.contextsleepnet.b2conv.fp8\endcsname{8.6}
\expandafter\def\csname v@gemm.contextsleepnet.b2conv.mkn\endcsname{15616\times448\times64}
\expandafter\def\csname v@gemm.contextsleepnet.b3conv.bf16\endcsname{8.2}
\expandafter\def\csname v@gemm.contextsleepnet.b3conv.fp32\endcsname{41.0}
\expandafter\def\csname v@gemm.contextsleepnet.b3conv.fp8\endcsname{8.6}
\expandafter\def\csname v@gemm.contextsleepnet.b3conv.mkn\endcsname{15616\times448\times64}
\expandafter\def\csname v@gemm.sleepcnn.conv1.bf16\endcsname{16.4}
\expandafter\def\csname v@gemm.sleepcnn.conv1.fp32\endcsname{26.7}
\expandafter\def\csname v@gemm.sleepcnn.conv1.fp8\endcsname{10.3}
\expandafter\def\csname v@gemm.sleepcnn.conv1.mkn\endcsname{151296\times64\times16}
\expandafter\def\csname v@gemm.sleepcnn.conv2.bf16\endcsname{6.2}
\expandafter\def\csname v@gemm.sleepcnn.conv2.fp32\endcsname{22.6}
\expandafter\def\csname v@gemm.sleepcnn.conv2.fp8\endcsname{8.7}
\expandafter\def\csname v@gemm.sleepcnn.conv2.mkn\endcsname{10496\times400\times32}
\expandafter\def\csname v@gemm.sleepcnn.fc1.bf16\endcsname{5.8}
\expandafter\def\csname v@gemm.sleepcnn.fc1.fp32\endcsname{12.3}
\expandafter\def\csname v@gemm.sleepcnn.fc1.fp8\endcsname{8.6}
\expandafter\def\csname v@gemm.sleepcnn.fc1.mkn\endcsname{256\times320\times128}
\expandafter\def\csname v@hw.cnn.bfloat16.lat\endcsname{0.038}
\expandafter\def\csname v@hw.cnn.bfloat16.latng\endcsname{0.088}
\expandafter\def\csname v@hw.cnn.bfloat16.tput\endcsname{4.34}
\expandafter\def\csname v@hw.cnn.bfloat16.uj\endcsname{39.8}
\expandafter\def\csname v@hw.cnn.float16.lat\endcsname{0.039}
\expandafter\def\csname v@hw.cnn.float16.latng\endcsname{0.087}
\expandafter\def\csname v@hw.cnn.float16.tput\endcsname{4.50}
\expandafter\def\csname v@hw.cnn.float16.uj\endcsname{38.8}
\expandafter\def\csname v@hw.cnn.float32.lat\endcsname{0.041}
\expandafter\def\csname v@hw.cnn.float32.latng\endcsname{0.077}
\expandafter\def\csname v@hw.cnn.float32.tput\endcsname{3.14}
\expandafter\def\csname v@hw.cnn.float32.uj\endcsname{76.1}
\expandafter\def\csname v@hw.cnn.graphx\endcsname{1.9}
\expandafter\def\csname v@hw.cnn.nmax\endcsname{256}
\expandafter\def\csname v@hw.cnn.nmin\endcsname{1}
\expandafter\def\csname v@hw.cnn.tputx\endcsname{1.4}
\expandafter\def\csname v@hw.cnn.ujx\endcsname{2.0}
\expandafter\def\csname v@hw.ctx.bfloat16.lat\endcsname{0.120}
\expandafter\def\csname v@hw.ctx.bfloat16.latng\endcsname{0.289}
\expandafter\def\csname v@hw.ctx.bfloat16.tput\endcsname{2.59}
\expandafter\def\csname v@hw.ctx.bfloat16.uj\endcsname{124.7}
\expandafter\def\csname v@hw.ctx.float16.lat\endcsname{0.118}
\expandafter\def\csname v@hw.ctx.float16.latng\endcsname{0.284}
\expandafter\def\csname v@hw.ctx.float16.tput\endcsname{2.63}
\expandafter\def\csname v@hw.ctx.float16.uj\endcsname{125.6}
\expandafter\def\csname v@hw.ctx.float32.lat\endcsname{0.180}
\expandafter\def\csname v@hw.ctx.float32.latng\endcsname{0.236}
\expandafter\def\csname v@hw.ctx.float32.tput\endcsname{1.07}
\expandafter\def\csname v@hw.ctx.float32.uj\endcsname{259.2}
\expandafter\def\csname v@hw.ctx.graphx\endcsname{1.3}
\expandafter\def\csname v@hw.ctx.nmax\endcsname{1024}
\expandafter\def\csname v@hw.ctx.nmin\endcsname{31}
\expandafter\def\csname v@hw.ctx.tputx\endcsname{2.5}
\expandafter\def\csname v@hw.ctx.ujx\endcsname{2.1}
\expandafter\def\csname v@hw.rep.energy\endcsname{33}
\expandafter\def\csname v@hw.rep.n\endcsname{three}
\expandafter\def\csname v@hw.rep.perf\endcsname{12}
\expandafter\def\csname v@int4.bits\endcsname{5.125}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.a.d\endcsname{\mns{}0.86}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.a.hi\endcsname{\mns{}0.45}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.a.lo\endcsname{\mns{}1.30}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.a.med\endcsname{\mns{}0.54}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.a.p\endcsname{<0.001}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.a.ph\endcsname{0.004}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.w.d\endcsname{\mns{}0.97}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.w.hi\endcsname{\mns{}0.60}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.w.lo\endcsname{\mns{}1.34}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.w.med\endcsname{\mns{}0.69}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.w.p\endcsname{<0.001}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.w.ph\endcsname{<0.001}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.wa.d\endcsname{\mns{}2.35}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.wa.hi\endcsname{\mns{}1.64}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.wa.lo\endcsname{\mns{}3.06}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.wa.med\endcsname{\mns{}1.47}
\expandafter\def\csname v@lone.cnn.mxfp432w4a4.wa.p\endcsname{<0.001}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.a.d\endcsname{\mns{}0.87}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.a.hi\endcsname{\mns{}0.50}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.a.lo\endcsname{\mns{}1.27}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.a.med\endcsname{\mns{}0.57}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.a.p\endcsname{<0.001}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.a.ph\endcsname{0.001}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.w.d\endcsname{\mns{}0.49}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.w.hi\endcsname{\mns{}0.21}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.w.lo\endcsname{\mns{}0.77}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.w.med\endcsname{\mns{}0.37}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.w.p\endcsname{<0.001}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.w.ph\endcsname{0.003}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.wa.d\endcsname{\mns{}1.71}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.wa.hi\endcsname{\mns{}1.17}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.wa.lo\endcsname{\mns{}2.28}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.wa.med\endcsname{\mns{}1.27}
\expandafter\def\csname v@lone.cnn.nvfp416w4a4.wa.p\endcsname{<0.001}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.a.d\endcsname{\mns{}0.07}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.a.hi\endcsname{\pls{}0.20}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.a.lo\endcsname{\mns{}0.37}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.a.med\endcsname{\pls{}0.23}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.a.p\endcsname{0.83}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.a.ph\endcsname{1.00}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.w.d\endcsname{\mns{}0.04}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.w.hi\endcsname{\pls{}0.21}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.w.lo\endcsname{\mns{}0.33}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.w.med\endcsname{\pls{}0.06}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.w.p\endcsname{0.73}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.w.ph\endcsname{1.00}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.wa.d\endcsname{\mns{}0.45}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.wa.hi\endcsname{\pls{}0.06}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.wa.lo\endcsname{\mns{}1.01}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.wa.med\endcsname{\mns{}0.11}
\expandafter\def\csname v@lone.ctx.mxfp432w4a4.wa.p\endcsname{0.20}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.a.d\endcsname{\mns{}0.07}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.a.hi\endcsname{\pls{}0.18}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.a.lo\endcsname{\mns{}0.32}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.a.med\endcsname{\pls{}0.18}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.a.p\endcsname{0.91}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.a.ph\endcsname{1.00}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.w.d\endcsname{\mns{}0.09}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.w.hi\endcsname{\pls{}0.07}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.w.lo\endcsname{\mns{}0.27}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.w.med\endcsname{\pls{}0.02}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.w.p\endcsname{0.61}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.w.ph\endcsname{1.00}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.wa.d\endcsname{\mns{}0.40}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.wa.hi\endcsname{\pls{}0.00}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.wa.lo\endcsname{\mns{}0.79}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.wa.med\endcsname{\mns{}0.12}
\expandafter\def\csname v@lone.ctx.nvfp416w4a4.wa.p\endcsname{0.13}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.a.d\endcsname{\mns{}0.22}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.a.hi\endcsname{\pls{}0.13}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.a.lo\endcsname{\mns{}0.59}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.a.med\endcsname{\pls{}0.13}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.a.p\endcsname{0.35}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.a.ph\endcsname{1.00}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.w.d\endcsname{\mns{}0.24}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.w.hi\endcsname{\pls{}0.13}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.w.lo\endcsname{\mns{}0.65}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.w.med\endcsname{\pls{}0.14}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.w.p\endcsname{0.69}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.w.ph\endcsname{1.00}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.wa.d\endcsname{\mns{}1.05}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.wa.hi\endcsname{\mns{}0.32}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.wa.lo\endcsname{\mns{}1.79}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.wa.med\endcsname{\mns{}0.10}
\expandafter\def\csname v@lone.enc.mxfp432w4a4.wa.p\endcsname{0.04}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.a.d\endcsname{\mns{}0.19}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.a.hi\endcsname{\pls{}0.14}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.a.lo\endcsname{\mns{}0.52}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.a.med\endcsname{\pls{}0.11}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.a.p\endcsname{0.42}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.a.ph\endcsname{1.00}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.w.d\endcsname{\mns{}0.17}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.w.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.w.lo\endcsname{\mns{}0.36}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.w.med\endcsname{\mns{}0.00}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.w.p\endcsname{0.22}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.w.ph\endcsname{1.00}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.wa.d\endcsname{\mns{}0.57}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.wa.hi\endcsname{\mns{}0.08}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.wa.lo\endcsname{\mns{}1.07}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.wa.med\endcsname{\mns{}0.27}
\expandafter\def\csname v@lone.enc.nvfp416w4a4.wa.p\endcsname{0.07}
\expandafter\def\csname v@mix.maxabs\endcsname{0.48}
\expandafter\def\csname v@mix.ovhmax\endcsname{2.1}
\expandafter\def\csname v@mix.ovhmin\endcsname{0.7}
\expandafter\def\csname v@nat.agree.min\endcsname{99.83}
\expandafter\def\csname v@nat.cnn.bf16.agree\endcsname{99.83}
\expandafter\def\csname v@nat.cnn.fp16.agree\endcsname{99.98}
\expandafter\def\csname v@nat.ctx.bf16.agree\endcsname{99.87}
\expandafter\def\csname v@nat.ctx.fp16.agree\endcsname{99.99}
\expandafter\def\csname v@nat.diff.max\endcsname{0.023}
\expandafter\def\csname v@ni.cnn.bf16.hi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ni.cnn.bf16.lo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ni.cnn.bf16.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.fl.lomin\endcsname{\mns{}0.68}
\expandafter\def\csname v@ni.cnn.fp16.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ni.cnn.fp16.lo\endcsname{\mns{}0.00}
\expandafter\def\csname v@ni.cnn.fp16.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.fp32ft.hi\endcsname{\pls{}0.69}
\expandafter\def\csname v@ni.cnn.fp32ft.lo\endcsname{\mns{}0.18}
\expandafter\def\csname v@ni.cnn.fp32ft.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.fp8e4m3w8a8.hi\endcsname{\mns{}0.01}
\expandafter\def\csname v@ni.cnn.fp8e4m3w8a8.lo\endcsname{\mns{}0.26}
\expandafter\def\csname v@ni.cnn.fp8e4m3w8a8.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.fp8e5m2w8a8.hi\endcsname{\mns{}0.14}
\expandafter\def\csname v@ni.cnn.fp8e5m2w8a8.lo\endcsname{\mns{}0.79}
\expandafter\def\csname v@ni.cnn.fp8e5m2w8a8.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.int4g32w4.hi\endcsname{\mns{}0.27}
\expandafter\def\csname v@ni.cnn.int4g32w4.lo\endcsname{\mns{}0.98}
\expandafter\def\csname v@ni.cnn.int4g32w4.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.int8w8.hi\endcsname{\pls{}0.07}
\expandafter\def\csname v@ni.cnn.int8w8.lo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ni.cnn.int8w8.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.int8w8a8.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@ni.cnn.int8w8a8.lo\endcsname{\mns{}0.16}
\expandafter\def\csname v@ni.cnn.int8w8a8.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.mxfp416w4a4.hi\endcsname{\mns{}1.96}
\expandafter\def\csname v@ni.cnn.mxfp416w4a4.lo\endcsname{\mns{}4.12}
\expandafter\def\csname v@ni.cnn.mxfp416w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.cnn.mxfp432w4.hi\endcsname{\mns{}0.76}
\expandafter\def\csname v@ni.cnn.mxfp432w4.lo\endcsname{\mns{}1.85}
\expandafter\def\csname v@ni.cnn.mxfp432w4.ok\endcsname{no}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4.hi\endcsname{\mns{}2.01}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4.lo\endcsname{\mns{}4.11}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4fp8first.hi\endcsname{\mns{}0.44}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4fp8first.lo\endcsname{\mns{}0.97}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4fp8first.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4fp8firstlast.hi\endcsname{\mns{}0.28}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.68}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4fp8firstlast.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4qat.hi\endcsname{\pls{}0.17}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4qat.lo\endcsname{\mns{}0.71}
\expandafter\def\csname v@ni.cnn.mxfp432w4a4qat.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.nvfp416w4.hi\endcsname{\mns{}0.23}
\expandafter\def\csname v@ni.cnn.nvfp416w4.lo\endcsname{\mns{}1.12}
\expandafter\def\csname v@ni.cnn.nvfp416w4.ok\endcsname{no}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4.hi\endcsname{\mns{}1.20}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4.lo\endcsname{\mns{}2.79}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4fp8first.hi\endcsname{\mns{}0.18}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4fp8first.lo\endcsname{\mns{}0.51}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4fp8first.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4fp8firstlast.hi\endcsname{\mns{}0.09}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.41}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4fp8firstlast.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4qat.hi\endcsname{\pls{}0.18}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4qat.lo\endcsname{\mns{}0.77}
\expandafter\def\csname v@ni.cnn.nvfp416w4a4qat.ok\endcsname{yes}
\expandafter\def\csname v@ni.cnn.nvfp432w4a4.hi\endcsname{\mns{}1.53}
\expandafter\def\csname v@ni.cnn.nvfp432w4a4.lo\endcsname{\mns{}3.33}
\expandafter\def\csname v@ni.cnn.nvfp432w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.cnn.wfour.lomax\endcsname{\mns{}2.79}
\expandafter\def\csname v@ni.cnn.wfour.lomin\endcsname{\mns{}4.12}
\expandafter\def\csname v@ni.ctx.bf16.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@ni.ctx.bf16.lo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ni.ctx.bf16.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.fl.lomin\endcsname{\mns{}0.52}
\expandafter\def\csname v@ni.ctx.fp16.hi\endcsname{\pls{}0.00}
\expandafter\def\csname v@ni.ctx.fp16.lo\endcsname{\mns{}0.00}
\expandafter\def\csname v@ni.ctx.fp16.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.fp32ft.hi\endcsname{\pls{}0.94}
\expandafter\def\csname v@ni.ctx.fp32ft.lo\endcsname{\mns{}0.17}
\expandafter\def\csname v@ni.ctx.fp32ft.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.fp8e4m3w8a8.hi\endcsname{\pls{}0.11}
\expandafter\def\csname v@ni.ctx.fp8e4m3w8a8.lo\endcsname{\mns{}0.07}
\expandafter\def\csname v@ni.ctx.fp8e4m3w8a8.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.fp8e5m2w8a8.hi\endcsname{\pls{}0.23}
\expandafter\def\csname v@ni.ctx.fp8e5m2w8a8.lo\endcsname{\mns{}0.16}
\expandafter\def\csname v@ni.ctx.fp8e5m2w8a8.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.int4g32w4.hi\endcsname{\pls{}0.20}
\expandafter\def\csname v@ni.ctx.int4g32w4.lo\endcsname{\mns{}0.17}
\expandafter\def\csname v@ni.ctx.int4g32w4.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.int8w8.hi\endcsname{\pls{}0.03}
\expandafter\def\csname v@ni.ctx.int8w8.lo\endcsname{\mns{}0.02}
\expandafter\def\csname v@ni.ctx.int8w8.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.int8w8a8.hi\endcsname{\pls{}0.04}
\expandafter\def\csname v@ni.ctx.int8w8a8.lo\endcsname{\mns{}0.11}
\expandafter\def\csname v@ni.ctx.int8w8a8.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.mxfp416w4a4.hi\endcsname{\mns{}0.27}
\expandafter\def\csname v@ni.ctx.mxfp416w4a4.lo\endcsname{\mns{}2.20}
\expandafter\def\csname v@ni.ctx.mxfp416w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.ctx.mxfp432w4.hi\endcsname{\pls{}0.28}
\expandafter\def\csname v@ni.ctx.mxfp432w4.lo\endcsname{\mns{}0.68}
\expandafter\def\csname v@ni.ctx.mxfp432w4.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4.hi\endcsname{\mns{}0.09}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4.lo\endcsname{\mns{}1.82}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4fp8first.hi\endcsname{\pls{}0.15}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4fp8first.lo\endcsname{\mns{}0.66}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4fp8first.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.22}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.52}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4fp8firstlast.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4qat.hi\endcsname{\pls{}0.70}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4qat.lo\endcsname{\mns{}0.34}
\expandafter\def\csname v@ni.ctx.mxfp432w4a4qat.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.nvfp416w4.hi\endcsname{\pls{}0.13}
\expandafter\def\csname v@ni.ctx.nvfp416w4.lo\endcsname{\mns{}0.42}
\expandafter\def\csname v@ni.ctx.nvfp416w4.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4.hi\endcsname{\pls{}0.11}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4.lo\endcsname{\mns{}1.11}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4fp8first.hi\endcsname{\pls{}0.21}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4fp8first.lo\endcsname{\mns{}0.17}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4fp8first.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.19}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.09}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4fp8firstlast.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4qat.hi\endcsname{\pls{}0.98}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4qat.lo\endcsname{\mns{}0.13}
\expandafter\def\csname v@ni.ctx.nvfp416w4a4qat.ok\endcsname{yes}
\expandafter\def\csname v@ni.ctx.nvfp432w4a4.hi\endcsname{\pls{}0.25}
\expandafter\def\csname v@ni.ctx.nvfp432w4a4.lo\endcsname{\mns{}1.09}
\expandafter\def\csname v@ni.ctx.nvfp432w4a4.ok\endcsname{no}
\expandafter\def\csname v@ni.ctx.wfour.lomax\endcsname{\mns{}1.09}
\expandafter\def\csname v@ni.ctx.wfour.lomin\endcsname{\mns{}2.20}
\expandafter\def\csname v@ni.eightbit.minlo\endcsname{\mns{}0.79}
\expandafter\def\csname v@ni.fl.lomin\endcsname{\mns{}0.68}
\expandafter\def\csname v@ni.level\endcsname{0.0025}
\expandafter\def\csname v@ni.m\endcsname{20}
\expandafter\def\csname v@ni.margin\endcsname{1}
\expandafter\def\csname v@ni.qat.lomin\endcsname{\mns{}0.77}
\expandafter\def\csname v@nirob.int4.bca\endcsname{\mns{}1.011}
\expandafter\def\csname v@nirob.int4.percentile\endcsname{\mns{}0.983}
\expandafter\def\csname v@nirob.int4.seedsmax\endcsname{\mns{}0.974}
\expandafter\def\csname v@nirob.int4.seedsmin\endcsname{\mns{}0.997}
\expandafter\def\csname v@nirob.int4.t\endcsname{\mns{}0.987}
\expandafter\def\csname v@nirob.n\endcsname{40}
\expandafter\def\csname v@nirob.same\endcsname{39}
\expandafter\def\csname v@run.download\endcsname{140}
\expandafter\def\csname v@run.minutes\endcsname{89.0}
\expandafter\def\csname v@sc20.cnn.bf16.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@sc20.cnn.bf16.hi\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.cnn.bf16.lo\endcsname{\mns{}0.05}
\expandafter\def\csname v@sc20.cnn.bf16.med\endcsname{\mns{}0.01}
\expandafter\def\csname v@sc20.cnn.bf16.p\endcsname{0.08}
\expandafter\def\csname v@sc20.cnn.bf16.ph\endcsname{0.41}
\expandafter\def\csname v@sc20.cnn.fp16.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.cnn.fp16.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.cnn.fp16.lo\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.cnn.fp16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.cnn.fp16.p\endcsname{0.02}
\expandafter\def\csname v@sc20.cnn.fp16.ph\endcsname{0.18}
\expandafter\def\csname v@sc20.cnn.fp32.acc\endcsname{78.6}
\expandafter\def\csname v@sc20.cnn.fp32.kappa\endcsname{0.713}
\expandafter\def\csname v@sc20.cnn.fp32.mf1\endcsname{73.2}
\expandafter\def\csname v@sc20.cnn.fp32.mf1sd\endcsname{0.45}
\expandafter\def\csname v@sc20.cnn.fp8e4m3w8a8.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.cnn.fp8e4m3w8a8.hi\endcsname{\pls{}0.19}
\expandafter\def\csname v@sc20.cnn.fp8e4m3w8a8.lo\endcsname{\mns{}0.17}
\expandafter\def\csname v@sc20.cnn.fp8e4m3w8a8.med\endcsname{\pls{}0.03}
\expandafter\def\csname v@sc20.cnn.fp8e4m3w8a8.p\endcsname{0.50}
\expandafter\def\csname v@sc20.cnn.fp8e4m3w8a8.ph\endcsname{0.71}
\expandafter\def\csname v@sc20.cnn.fp8e5m2w8a8.d\endcsname{\mns{}0.27}
\expandafter\def\csname v@sc20.cnn.fp8e5m2w8a8.hi\endcsname{\mns{}0.07}
\expandafter\def\csname v@sc20.cnn.fp8e5m2w8a8.lo\endcsname{\mns{}0.46}
\expandafter\def\csname v@sc20.cnn.fp8e5m2w8a8.med\endcsname{\mns{}0.28}
\expandafter\def\csname v@sc20.cnn.fp8e5m2w8a8.p\endcsname{0.02}
\expandafter\def\csname v@sc20.cnn.fp8e5m2w8a8.ph\endcsname{0.17}
\expandafter\def\csname v@sc20.cnn.int4g32w4.d\endcsname{\mns{}0.38}
\expandafter\def\csname v@sc20.cnn.int4g32w4.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.cnn.int4g32w4.lo\endcsname{\mns{}0.85}
\expandafter\def\csname v@sc20.cnn.int4g32w4.med\endcsname{\mns{}0.35}
\expandafter\def\csname v@sc20.cnn.int4g32w4.p\endcsname{0.05}
\expandafter\def\csname v@sc20.cnn.int4g32w4.ph\endcsname{0.31}
\expandafter\def\csname v@sc20.cnn.int8w8.d\endcsname{\mns{}0.02}
\expandafter\def\csname v@sc20.cnn.int8w8.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.cnn.int8w8.lo\endcsname{\mns{}0.05}
\expandafter\def\csname v@sc20.cnn.int8w8.med\endcsname{\mns{}0.03}
\expandafter\def\csname v@sc20.cnn.int8w8.p\endcsname{0.18}
\expandafter\def\csname v@sc20.cnn.int8w8.ph\endcsname{0.71}
\expandafter\def\csname v@sc20.cnn.int8w8a8.d\endcsname{\mns{}0.15}
\expandafter\def\csname v@sc20.cnn.int8w8a8.hi\endcsname{\mns{}0.06}
\expandafter\def\csname v@sc20.cnn.int8w8a8.lo\endcsname{\mns{}0.25}
\expandafter\def\csname v@sc20.cnn.int8w8a8.med\endcsname{\mns{}0.18}
\expandafter\def\csname v@sc20.cnn.int8w8a8.p\endcsname{0.006}
\expandafter\def\csname v@sc20.cnn.int8w8a8.ph\endcsname{0.07}
\expandafter\def\csname v@sc20.cnn.mxfp416w4a4.d\endcsname{\mns{}1.67}
\expandafter\def\csname v@sc20.cnn.mxfp416w4a4.hi\endcsname{\mns{}0.49}
\expandafter\def\csname v@sc20.cnn.mxfp416w4a4.lo\endcsname{\mns{}2.83}
\expandafter\def\csname v@sc20.cnn.mxfp416w4a4.med\endcsname{\mns{}1.79}
\expandafter\def\csname v@sc20.cnn.mxfp416w4a4.p\endcsname{0.004}
\expandafter\def\csname v@sc20.cnn.mxfp416w4a4.ph\endcsname{0.05}
\expandafter\def\csname v@sc20.cnn.mxfp432w4.d\endcsname{\mns{}0.45}
\expandafter\def\csname v@sc20.cnn.mxfp432w4.hi\endcsname{\pls{}0.21}
\expandafter\def\csname v@sc20.cnn.mxfp432w4.lo\endcsname{\mns{}0.98}
\expandafter\def\csname v@sc20.cnn.mxfp432w4.med\endcsname{\mns{}0.55}
\expandafter\def\csname v@sc20.cnn.mxfp432w4.p\endcsname{0.006}
\expandafter\def\csname v@sc20.cnn.mxfp432w4.ph\endcsname{0.07}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4.d\endcsname{\mns{}1.42}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4.hi\endcsname{\mns{}0.32}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4.lo\endcsname{\mns{}2.51}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4.med\endcsname{\mns{}1.53}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4.p\endcsname{0.004}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4.ph\endcsname{0.05}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8first.d\endcsname{\mns{}0.40}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8first.hi\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8first.lo\endcsname{\mns{}0.78}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8first.med\endcsname{\mns{}0.49}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8first.p\endcsname{0.04}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8first.ph\endcsname{0.31}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.23}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8firstlast.hi\endcsname{\pls{}0.14}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}0.58}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.11}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8firstlast.p\endcsname{0.22}
\expandafter\def\csname v@sc20.cnn.mxfp432w4a4fp8firstlast.ph\endcsname{0.71}
\expandafter\def\csname v@sc20.cnn.nvfp416w4.d\endcsname{\mns{}0.69}
\expandafter\def\csname v@sc20.cnn.nvfp416w4.hi\endcsname{\mns{}0.36}
\expandafter\def\csname v@sc20.cnn.nvfp416w4.lo\endcsname{\mns{}1.05}
\expandafter\def\csname v@sc20.cnn.nvfp416w4.med\endcsname{\mns{}0.60}
\expandafter\def\csname v@sc20.cnn.nvfp416w4.p\endcsname{<0.001}
\expandafter\def\csname v@sc20.cnn.nvfp416w4.ph\endcsname{0.008}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4.d\endcsname{\mns{}1.37}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4.hi\endcsname{\mns{}0.75}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4.lo\endcsname{\mns{}2.08}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4.med\endcsname{\mns{}1.28}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4.ph\endcsname{0.008}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8first.d\endcsname{\mns{}0.33}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8first.hi\endcsname{\mns{}0.10}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8first.lo\endcsname{\mns{}0.57}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8first.med\endcsname{\mns{}0.25}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8first.p\endcsname{0.02}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8first.ph\endcsname{0.17}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8firstlast.d\endcsname{\mns{}0.17}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.38}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8firstlast.med\endcsname{\mns{}0.05}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8firstlast.p\endcsname{0.20}
\expandafter\def\csname v@sc20.cnn.nvfp416w4a4fp8firstlast.ph\endcsname{0.71}
\expandafter\def\csname v@sc20.cnn.nvfp432w4a4.d\endcsname{\mns{}1.59}
\expandafter\def\csname v@sc20.cnn.nvfp432w4a4.hi\endcsname{\mns{}0.84}
\expandafter\def\csname v@sc20.cnn.nvfp432w4a4.lo\endcsname{\mns{}2.38}
\expandafter\def\csname v@sc20.cnn.nvfp432w4a4.med\endcsname{\mns{}1.31}
\expandafter\def\csname v@sc20.cnn.nvfp432w4a4.p\endcsname{0.001}
\expandafter\def\csname v@sc20.cnn.nvfp432w4a4.ph\endcsname{0.02}
\expandafter\def\csname v@sc20.ctx.bf16.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.ctx.bf16.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.ctx.bf16.lo\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.ctx.bf16.med\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.ctx.bf16.p\endcsname{0.27}
\expandafter\def\csname v@sc20.ctx.bf16.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.fp16.d\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.ctx.fp16.hi\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.ctx.fp16.lo\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.ctx.fp16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.ctx.fp16.p\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.fp16.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.fp32.acc\endcsname{81.9}
\expandafter\def\csname v@sc20.ctx.fp32.kappa\endcsname{0.758}
\expandafter\def\csname v@sc20.ctx.fp32.mf1\endcsname{77.7}
\expandafter\def\csname v@sc20.ctx.fp32.mf1sd\endcsname{0.20}
\expandafter\def\csname v@sc20.ctx.fp8e4m3w8a8.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.ctx.fp8e4m3w8a8.hi\endcsname{\pls{}0.10}
\expandafter\def\csname v@sc20.ctx.fp8e4m3w8a8.lo\endcsname{\mns{}0.08}
\expandafter\def\csname v@sc20.ctx.fp8e4m3w8a8.med\endcsname{\mns{}0.02}
\expandafter\def\csname v@sc20.ctx.fp8e4m3w8a8.p\endcsname{0.78}
\expandafter\def\csname v@sc20.ctx.fp8e4m3w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.fp8e5m2w8a8.d\endcsname{\mns{}0.08}
\expandafter\def\csname v@sc20.ctx.fp8e5m2w8a8.hi\endcsname{\pls{}0.08}
\expandafter\def\csname v@sc20.ctx.fp8e5m2w8a8.lo\endcsname{\mns{}0.23}
\expandafter\def\csname v@sc20.ctx.fp8e5m2w8a8.med\endcsname{\mns{}0.12}
\expandafter\def\csname v@sc20.ctx.fp8e5m2w8a8.p\endcsname{0.19}
\expandafter\def\csname v@sc20.ctx.fp8e5m2w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.int4g32w4.d\endcsname{\mns{}0.09}
\expandafter\def\csname v@sc20.ctx.int4g32w4.hi\endcsname{\pls{}0.14}
\expandafter\def\csname v@sc20.ctx.int4g32w4.lo\endcsname{\mns{}0.35}
\expandafter\def\csname v@sc20.ctx.int4g32w4.med\endcsname{\mns{}0.15}
\expandafter\def\csname v@sc20.ctx.int4g32w4.p\endcsname{0.57}
\expandafter\def\csname v@sc20.ctx.int4g32w4.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.int8w8.d\endcsname{\mns{}0.03}
\expandafter\def\csname v@sc20.ctx.int8w8.hi\endcsname{\mns{}0.01}
\expandafter\def\csname v@sc20.ctx.int8w8.lo\endcsname{\mns{}0.05}
\expandafter\def\csname v@sc20.ctx.int8w8.med\endcsname{\mns{}0.03}
\expandafter\def\csname v@sc20.ctx.int8w8.p\endcsname{0.03}
\expandafter\def\csname v@sc20.ctx.int8w8.ph\endcsname{0.32}
\expandafter\def\csname v@sc20.ctx.int8w8a8.d\endcsname{\mns{}0.07}
\expandafter\def\csname v@sc20.ctx.int8w8a8.hi\endcsname{\mns{}0.01}
\expandafter\def\csname v@sc20.ctx.int8w8a8.lo\endcsname{\mns{}0.12}
\expandafter\def\csname v@sc20.ctx.int8w8a8.med\endcsname{\mns{}0.05}
\expandafter\def\csname v@sc20.ctx.int8w8a8.p\endcsname{0.07}
\expandafter\def\csname v@sc20.ctx.int8w8a8.ph\endcsname{0.77}
\expandafter\def\csname v@sc20.ctx.mxfp416w4a4.d\endcsname{\mns{}3.90}
\expandafter\def\csname v@sc20.ctx.mxfp416w4a4.hi\endcsname{\mns{}2.26}
\expandafter\def\csname v@sc20.ctx.mxfp416w4a4.lo\endcsname{\mns{}5.85}
\expandafter\def\csname v@sc20.ctx.mxfp416w4a4.med\endcsname{\mns{}3.59}
\expandafter\def\csname v@sc20.ctx.mxfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@sc20.ctx.mxfp416w4a4.ph\endcsname{0.001}
\expandafter\def\csname v@sc20.ctx.mxfp432w4.d\endcsname{\mns{}1.22}
\expandafter\def\csname v@sc20.ctx.mxfp432w4.hi\endcsname{\mns{}0.46}
\expandafter\def\csname v@sc20.ctx.mxfp432w4.lo\endcsname{\mns{}2.13}
\expandafter\def\csname v@sc20.ctx.mxfp432w4.med\endcsname{\mns{}1.03}
\expandafter\def\csname v@sc20.ctx.mxfp432w4.p\endcsname{0.004}
\expandafter\def\csname v@sc20.ctx.mxfp432w4.ph\endcsname{0.06}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4.d\endcsname{\mns{}3.03}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4.hi\endcsname{\mns{}1.73}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4.lo\endcsname{\mns{}4.63}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4.med\endcsname{\mns{}2.71}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4.ph\endcsname{0.002}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8first.d\endcsname{\mns{}1.24}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8first.hi\endcsname{\mns{}0.47}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8first.lo\endcsname{\mns{}1.97}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8first.med\endcsname{\mns{}1.27}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8first.p\endcsname{0.006}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8first.ph\endcsname{0.07}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}1.12}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8firstlast.hi\endcsname{\mns{}0.41}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}1.77}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}1.06}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8firstlast.p\endcsname{0.002}
\expandafter\def\csname v@sc20.ctx.mxfp432w4a4fp8firstlast.ph\endcsname{0.03}
\expandafter\def\csname v@sc20.ctx.nvfp416w4.d\endcsname{\mns{}0.14}
\expandafter\def\csname v@sc20.ctx.nvfp416w4.hi\endcsname{\pls{}0.23}
\expandafter\def\csname v@sc20.ctx.nvfp416w4.lo\endcsname{\mns{}0.47}
\expandafter\def\csname v@sc20.ctx.nvfp416w4.med\endcsname{\mns{}0.23}
\expandafter\def\csname v@sc20.ctx.nvfp416w4.p\endcsname{0.28}
\expandafter\def\csname v@sc20.ctx.nvfp416w4.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4.hi\endcsname{\pls{}0.19}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4.lo\endcsname{\mns{}0.68}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4.med\endcsname{\mns{}0.36}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4.p\endcsname{0.25}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8first.d\endcsname{\mns{}0.01}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8first.hi\endcsname{\pls{}0.17}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8first.lo\endcsname{\mns{}0.18}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8first.med\endcsname{\mns{}0.04}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8first.p\endcsname{0.81}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8first.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8firstlast.d\endcsname{\pls{}0.03}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.16}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.09}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.03}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8firstlast.p\endcsname{0.67}
\expandafter\def\csname v@sc20.ctx.nvfp416w4a4fp8firstlast.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.ctx.nvfp432w4a4.d\endcsname{\mns{}0.51}
\expandafter\def\csname v@sc20.ctx.nvfp432w4a4.hi\endcsname{\pls{}0.11}
\expandafter\def\csname v@sc20.ctx.nvfp432w4a4.lo\endcsname{\mns{}1.15}
\expandafter\def\csname v@sc20.ctx.nvfp432w4a4.med\endcsname{\mns{}0.31}
\expandafter\def\csname v@sc20.ctx.nvfp432w4a4.p\endcsname{0.07}
\expandafter\def\csname v@sc20.ctx.nvfp432w4a4.ph\endcsname{0.77}
\expandafter\def\csname v@sc20.eightbit.maxabs\endcsname{0.27}
\expandafter\def\csname v@sc20.enc.bf16.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.enc.bf16.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.enc.bf16.lo\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.enc.bf16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.enc.bf16.p\endcsname{0.49}
\expandafter\def\csname v@sc20.enc.bf16.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.fp16.d\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.enc.fp16.hi\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.enc.fp16.lo\endcsname{\mns{}0.01}
\expandafter\def\csname v@sc20.enc.fp16.med\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.enc.fp16.p\endcsname{0.76}
\expandafter\def\csname v@sc20.enc.fp16.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.fp32.acc\endcsname{78.7}
\expandafter\def\csname v@sc20.enc.fp32.kappa\endcsname{0.715}
\expandafter\def\csname v@sc20.enc.fp32.mf1\endcsname{73.2}
\expandafter\def\csname v@sc20.enc.fp32.mf1sd\endcsname{0.15}
\expandafter\def\csname v@sc20.enc.fp8e4m3w8a8.d\endcsname{\pls{}0.01}
\expandafter\def\csname v@sc20.enc.fp8e4m3w8a8.hi\endcsname{\pls{}0.12}
\expandafter\def\csname v@sc20.enc.fp8e4m3w8a8.lo\endcsname{\mns{}0.09}
\expandafter\def\csname v@sc20.enc.fp8e4m3w8a8.med\endcsname{\mns{}0.01}
\expandafter\def\csname v@sc20.enc.fp8e4m3w8a8.p\endcsname{0.81}
\expandafter\def\csname v@sc20.enc.fp8e4m3w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.fp8e5m2w8a8.d\endcsname{\mns{}0.12}
\expandafter\def\csname v@sc20.enc.fp8e5m2w8a8.hi\endcsname{\pls{}0.17}
\expandafter\def\csname v@sc20.enc.fp8e5m2w8a8.lo\endcsname{\mns{}0.38}
\expandafter\def\csname v@sc20.enc.fp8e5m2w8a8.med\endcsname{\mns{}0.21}
\expandafter\def\csname v@sc20.enc.fp8e5m2w8a8.p\endcsname{0.18}
\expandafter\def\csname v@sc20.enc.fp8e5m2w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.int4g32w4.d\endcsname{\mns{}0.20}
\expandafter\def\csname v@sc20.enc.int4g32w4.hi\endcsname{\pls{}0.08}
\expandafter\def\csname v@sc20.enc.int4g32w4.lo\endcsname{\mns{}0.48}
\expandafter\def\csname v@sc20.enc.int4g32w4.med\endcsname{\mns{}0.21}
\expandafter\def\csname v@sc20.enc.int4g32w4.p\endcsname{0.18}
\expandafter\def\csname v@sc20.enc.int4g32w4.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.int8w8.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.enc.int8w8.hi\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.enc.int8w8.lo\endcsname{\mns{}0.03}
\expandafter\def\csname v@sc20.enc.int8w8.med\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.enc.int8w8.p\endcsname{0.39}
\expandafter\def\csname v@sc20.enc.int8w8.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.int8w8a8.d\endcsname{\pls{}0.00}
\expandafter\def\csname v@sc20.enc.int8w8a8.hi\endcsname{\pls{}0.07}
\expandafter\def\csname v@sc20.enc.int8w8a8.lo\endcsname{\mns{}0.07}
\expandafter\def\csname v@sc20.enc.int8w8a8.med\endcsname{\mns{}0.02}
\expandafter\def\csname v@sc20.enc.int8w8a8.p\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.int8w8a8.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.mxfp416w4a4.d\endcsname{\mns{}2.69}
\expandafter\def\csname v@sc20.enc.mxfp416w4a4.hi\endcsname{\mns{}1.60}
\expandafter\def\csname v@sc20.enc.mxfp416w4a4.lo\endcsname{\mns{}3.78}
\expandafter\def\csname v@sc20.enc.mxfp416w4a4.med\endcsname{\mns{}2.78}
\expandafter\def\csname v@sc20.enc.mxfp416w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@sc20.enc.mxfp416w4a4.ph\endcsname{0.004}
\expandafter\def\csname v@sc20.enc.mxfp432w4.d\endcsname{\mns{}0.78}
\expandafter\def\csname v@sc20.enc.mxfp432w4.hi\endcsname{\mns{}0.32}
\expandafter\def\csname v@sc20.enc.mxfp432w4.lo\endcsname{\mns{}1.28}
\expandafter\def\csname v@sc20.enc.mxfp432w4.med\endcsname{\mns{}0.64}
\expandafter\def\csname v@sc20.enc.mxfp432w4.p\endcsname{0.003}
\expandafter\def\csname v@sc20.enc.mxfp432w4.ph\endcsname{0.04}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4.d\endcsname{\mns{}2.32}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4.hi\endcsname{\mns{}1.31}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4.lo\endcsname{\mns{}3.31}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4.med\endcsname{\mns{}2.26}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4.p\endcsname{<0.001}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4.ph\endcsname{0.006}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8first.d\endcsname{\mns{}0.52}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8first.hi\endcsname{\mns{}0.16}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8first.lo\endcsname{\mns{}0.89}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8first.med\endcsname{\mns{}0.43}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8first.p\endcsname{0.02}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8first.ph\endcsname{0.24}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8firstlast.d\endcsname{\mns{}0.65}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8firstlast.hi\endcsname{\mns{}0.28}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8firstlast.lo\endcsname{\mns{}1.03}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8firstlast.med\endcsname{\mns{}0.55}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8firstlast.p\endcsname{0.002}
\expandafter\def\csname v@sc20.enc.mxfp432w4a4fp8firstlast.ph\endcsname{0.03}
\expandafter\def\csname v@sc20.enc.nvfp416w4.d\endcsname{\mns{}0.25}
\expandafter\def\csname v@sc20.enc.nvfp416w4.hi\endcsname{\pls{}0.21}
\expandafter\def\csname v@sc20.enc.nvfp416w4.lo\endcsname{\mns{}0.71}
\expandafter\def\csname v@sc20.enc.nvfp416w4.med\endcsname{\mns{}0.16}
\expandafter\def\csname v@sc20.enc.nvfp416w4.p\endcsname{0.22}
\expandafter\def\csname v@sc20.enc.nvfp416w4.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4.d\endcsname{\mns{}0.89}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4.hi\endcsname{\mns{}0.08}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4.lo\endcsname{\mns{}1.65}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4.med\endcsname{\mns{}0.94}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4.p\endcsname{0.02}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4.ph\endcsname{0.18}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8first.d\endcsname{\mns{}0.16}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8first.hi\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8first.lo\endcsname{\mns{}0.33}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8first.med\endcsname{\mns{}0.11}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8first.p\endcsname{0.11}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8first.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8firstlast.d\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8firstlast.hi\endcsname{\pls{}0.15}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8firstlast.lo\endcsname{\mns{}0.16}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8firstlast.med\endcsname{\pls{}0.02}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8firstlast.p\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.nvfp416w4a4fp8firstlast.ph\endcsname{1.00}
\expandafter\def\csname v@sc20.enc.nvfp432w4a4.d\endcsname{\mns{}1.07}
\expandafter\def\csname v@sc20.enc.nvfp432w4a4.hi\endcsname{\mns{}0.33}
\expandafter\def\csname v@sc20.enc.nvfp432w4a4.lo\endcsname{\mns{}1.74}
\expandafter\def\csname v@sc20.enc.nvfp432w4a4.med\endcsname{\mns{}1.28}
\expandafter\def\csname v@sc20.enc.nvfp432w4a4.p\endcsname{0.006}
\expandafter\def\csname v@sc20.enc.nvfp432w4a4.ph\endcsname{0.08}
\expandafter\def\csname v@sc20.tcn.mxfp416w4a4.d\endcsname{\mns{}1.21}
\expandafter\def\csname v@sc20.tcn.mxfp416w4a4.hi\endcsname{\mns{}0.04}
\expandafter\def\csname v@sc20.tcn.mxfp416w4a4.lo\endcsname{\mns{}2.61}
\expandafter\def\csname v@sc20.tcn.mxfp416w4a4.med\endcsname{\mns{}0.71}
\expandafter\def\csname v@sc20.tcn.mxfp416w4a4.p\endcsname{0.18}
\expandafter\def\csname v@sc20.tcn.mxfp416w4a4.ph\endcsname{0.35}
\expandafter\def\csname v@sc20.tcn.mxfp432w4a4.d\endcsname{\mns{}0.71}
\expandafter\def\csname v@sc20.tcn.mxfp432w4a4.hi\endcsname{\pls{}0.20}
\expandafter\def\csname v@sc20.tcn.mxfp432w4a4.lo\endcsname{\mns{}1.80}
\expandafter\def\csname v@sc20.tcn.mxfp432w4a4.med\endcsname{\mns{}0.00}
\expandafter\def\csname v@sc20.tcn.mxfp432w4a4.p\endcsname{0.45}
\expandafter\def\csname v@sc20.tcn.mxfp432w4a4.ph\endcsname{0.45}
\expandafter\def\csname v@sc20.tcn.nvfp416w4a4.d\endcsname{\pls{}0.64}
\expandafter\def\csname v@sc20.tcn.nvfp416w4a4.hi\endcsname{\pls{}1.11}
\expandafter\def\csname v@sc20.tcn.nvfp416w4a4.lo\endcsname{\pls{}0.12}
\expandafter\def\csname v@sc20.tcn.nvfp416w4a4.med\endcsname{\pls{}0.60}
\expandafter\def\csname v@sc20.tcn.nvfp416w4a4.p\endcsname{0.008}
\expandafter\def\csname v@sc20.tcn.nvfp416w4a4.ph\endcsname{0.03}
\expandafter\def\csname v@sc20.tcn.nvfp432w4a4.d\endcsname{\pls{}0.56}
\expandafter\def\csname v@sc20.tcn.nvfp432w4a4.hi\endcsname{\pls{}0.99}
\expandafter\def\csname v@sc20.tcn.nvfp432w4a4.lo\endcsname{\pls{}0.15}
\expandafter\def\csname v@sc20.tcn.nvfp432w4a4.med\endcsname{\pls{}0.54}
\expandafter\def\csname v@sc20.tcn.nvfp432w4a4.p\endcsname{0.02}
\expandafter\def\csname v@sc20.tcn.nvfp432w4a4.ph\endcsname{0.05}
\expandafter\def\csname v@sc20.total\endcsname{42{,}307}
\expandafter\def\csname v@spec.bump.nII\endcsname{1.9}
\expandafter\def\csname v@spec.bump.nIII\endcsname{2.2}
\expandafter\def\csname v@spec.nIrem.maxdb\endcsname{1.9}
\expandafter\def\csname v@spec.wbeta.margin\endcsname{5.5}
\expandafter\def\csname v@tao.exact\endcsname{32}
\expandafter\def\csname v@tao.tested\endcsname{32}
\expandafter\def\csname v@tao.torch\endcsname{2.11.0}
\expandafter\def\csname v@tao.version\endcsname{0.18.0}
\expandafter\def\csname v@w4a4.cnn.range\endcsname{1.98--3.04}
\expandafter\def\csname v@w4a4.ctx.max\endcsname{1.19}
\makeatother


==> numbers_subject.tex <==
% AUTO-GENERATED by make_subject.py (exploratory subject-level analysis)
\makeatletter
\expandafter\def\csname v@cm.cnn.mx.nIIInII\endcsname{7.1}
\expandafter\def\csname v@cm.cnn.mx.nIIIrecall\endcsname{9.7}
\expandafter\def\csname v@cm.cnn.mx.nIInI\endcsname{8.5}
\expandafter\def\csname v@cm.cnn.mx.remnI\endcsname{6.9}
\expandafter\def\csname v@cm.cnn.nv.nIIInII\endcsname{5.4}
\expandafter\def\csname v@cm.cnn.nv.nIIIrecall\endcsname{7.8}
\expandafter\def\csname v@cm.cnn.nv.nIInI\endcsname{5.3}
\expandafter\def\csname v@cm.cnn.nv.remnI\endcsname{3.3}
\expandafter\def\csname v@cm.ctx.mx.nIIInII\endcsname{8.9}
\expandafter\def\csname v@cm.ctx.mx.nIIIrecall\endcsname{9.6}
\expandafter\def\csname v@cm.ctx.mx.nIInI\endcsname{2.1}
\expandafter\def\csname v@cm.ctx.mx.remnI\endcsname{1.5}
\expandafter\def\csname v@cm.ctx.nv.nIIInII\endcsname{4.6}
\expandafter\def\csname v@cm.ctx.nv.nIIIrecall\endcsname{5.2}
\expandafter\def\csname v@cm.ctx.nv.nIInI\endcsname{2.6}
\expandafter\def\csname v@cm.ctx.nv.remnI\endcsname{2.2}
\expandafter\def\csname v@cnn.fp32.nIIIsharepred\endcsname{8.7}
\expandafter\def\csname v@cnn.fp32.nIsharepred\endcsname{16.9}
\expandafter\def\csname v@cnn.mx.nIIIsharepred\endcsname{6.8}
\expandafter\def\csname v@cnn.nv.nIIIsharepred\endcsname{7.2}
\expandafter\def\csname v@ctx.fp32.nIIIsharepred\endcsname{9.6}
\expandafter\def\csname v@ctx.fp32.nIsharepred\endcsname{14.7}
\expandafter\def\csname v@ctx.mx.nIIIsharepred\endcsname{7.4}
\expandafter\def\csname v@ctx.nv.nIIIsharepred\endcsname{8.3}
\expandafter\def\csname v@eightbit.noefivemax\endcsname{0.13}
\expandafter\def\csname v@ls.cnn.othermax\endcsname{0.24}
\expandafter\def\csname v@subj.con.cnn.blockmx.d\endcsname{0.02}
\expandafter\def\csname v@subj.con.cnn.blockmx.hi\endcsname{0.20}
\expandafter\def\csname v@subj.con.cnn.blockmx.lo\endcsname{\mns{}0.17}
\expandafter\def\csname v@subj.con.cnn.blockmx.ph\endcsname{0.87}
\expandafter\def\csname v@subj.con.cnn.blocknv.d\endcsname{0.40}
\expandafter\def\csname v@subj.con.cnn.blocknv.hi\endcsname{0.70}
\expandafter\def\csname v@subj.con.cnn.blocknv.lo\endcsname{0.13}
\expandafter\def\csname v@subj.con.cnn.blocknv.ph\endcsname{0.04}
\expandafter\def\csname v@subj.con.cnn.scale16.d\endcsname{1.04}
\expandafter\def\csname v@subj.con.cnn.scale16.hi\endcsname{1.37}
\expandafter\def\csname v@subj.con.cnn.scale16.lo\endcsname{0.72}
\expandafter\def\csname v@subj.con.cnn.scale16.ph\endcsname{<0.001}
\expandafter\def\csname v@subj.con.cnn.scale32.d\endcsname{0.66}
\expandafter\def\csname v@subj.con.cnn.scale32.hi\endcsname{1.09}
\expandafter\def\csname v@subj.con.cnn.scale32.lo\endcsname{0.20}
\expandafter\def\csname v@subj.con.cnn.scale32.ph\endcsname{0.02}
\expandafter\def\csname v@subj.con.ctx.blockmx.d\endcsname{\mns{}0.29}
\expandafter\def\csname v@subj.con.ctx.blockmx.hi\endcsname{\mns{}0.15}
\expandafter\def\csname v@subj.con.ctx.blockmx.lo\endcsname{\mns{}0.43}
\expandafter\def\csname v@subj.con.ctx.blockmx.ph\endcsname{0.02}
\expandafter\def\csname v@subj.con.ctx.blocknv.d\endcsname{\mns{}0.10}
\expandafter\def\csname v@subj.con.ctx.blocknv.hi\endcsname{0.06}
\expandafter\def\csname v@subj.con.ctx.blocknv.lo\endcsname{\mns{}0.26}
\expandafter\def\csname v@subj.con.ctx.blocknv.ph\endcsname{0.20}
\expandafter\def\csname v@subj.con.ctx.scale16.d\endcsname{0.71}
\expandafter\def\csname v@subj.con.ctx.scale16.hi\endcsname{1.19}
\expandafter\def\csname v@subj.con.ctx.scale16.lo\endcsname{0.24}
\expandafter\def\csname v@subj.con.ctx.scale16.ph\endcsname{0.06}
\expandafter\def\csname v@subj.con.ctx.scale32.d\endcsname{0.52}
\expandafter\def\csname v@subj.con.ctx.scale32.hi\endcsname{0.87}
\expandafter\def\csname v@subj.con.ctx.scale32.lo\endcsname{0.18}
\expandafter\def\csname v@subj.con.ctx.scale32.ph\endcsname{0.04}
\expandafter\def\csname v@subj.mx.cnn.rbase\endcsname{0.32}
\expandafter\def\csname v@subj.mx.cnn.rbase.p\endcsname{0.005}
\expandafter\def\csname v@subj.mx.cnn.rnthree\endcsname{0.36}
\expandafter\def\csname v@subj.mx.cnn.rnthree.p\endcsname{0.001}
\expandafter\def\csname v@subj.mx.cnn.seedmax\endcsname{0.64}
\expandafter\def\csname v@subj.mx.cnn.seedmin\endcsname{0.57}
\expandafter\def\csname v@subj.mx.ctx.rbase\endcsname{0.30}
\expandafter\def\csname v@subj.mx.ctx.rbase.p\endcsname{0.009}
\expandafter\def\csname v@subj.mx.ctx.rnthree\endcsname{0.27}
\expandafter\def\csname v@subj.mx.ctx.rnthree.p\endcsname{0.02}
\expandafter\def\csname v@subj.mx.ctx.seedmax\endcsname{0.52}
\expandafter\def\csname v@subj.mx.ctx.seedmin\endcsname{0.40}
\expandafter\def\csname v@subj.mx.xmodel\endcsname{0.69}
\expandafter\def\csname v@subj.mx.xmodel.p\endcsname{<0.001}
\expandafter\def\csname v@subj.mx.xmodel.seedmax\endcsname{0.62}
\expandafter\def\csname v@subj.mx.xmodel.seedmin\endcsname{0.52}
\expandafter\def\csname v@subj.noise.xmodel.max\endcsname{0.13}
\expandafter\def\csname v@subj.noise.xmodel.min\endcsname{\mns{}0.24}
\expandafter\def\csname v@subj.nv.cnn.rbase\endcsname{0.30}
\expandafter\def\csname v@subj.nv.cnn.rbase.p\endcsname{0.007}
\expandafter\def\csname v@subj.nv.cnn.rnthree\endcsname{0.31}
\expandafter\def\csname v@subj.nv.cnn.rnthree.p\endcsname{0.005}
\expandafter\def\csname v@subj.nv.cnn.seedmax\endcsname{0.70}
\expandafter\def\csname v@subj.nv.cnn.seedmin\endcsname{0.57}
\expandafter\def\csname v@subj.nv.ctx.rbase\endcsname{0.26}
\expandafter\def\csname v@subj.nv.ctx.rbase.p\endcsname{0.02}
\expandafter\def\csname v@subj.nv.ctx.rnthree\endcsname{0.36}
\expandafter\def\csname v@subj.nv.ctx.rnthree.p\endcsname{0.001}
\expandafter\def\csname v@subj.nv.ctx.seedmax\endcsname{0.63}
\expandafter\def\csname v@subj.nv.ctx.seedmin\endcsname{0.38}
\expandafter\def\csname v@subj.nv.xmodel\endcsname{0.78}
\expandafter\def\csname v@subj.nv.xmodel.p\endcsname{<0.001}
\expandafter\def\csname v@subj.nv.xmodel.seedmax\endcsname{0.61}
\expandafter\def\csname v@subj.nv.xmodel.seedmin\endcsname{0.49}
\expandafter\def\csname v@subj.rbase.max\endcsname{0.32}
\expandafter\def\csname v@subj.rbase.min\endcsname{0.26}
\expandafter\def\csname v@subj.rbase.pmax\endcsname{0.02}
\expandafter\def\csname v@subj.rnthree.max\endcsname{0.36}
\expandafter\def\csname v@subj.rnthree.min\endcsname{0.27}
\expandafter\def\csname v@subj.rnthree.pmax\endcsname{0.02}
\expandafter\def\csname v@subj.seed.max\endcsname{0.70}
\expandafter\def\csname v@subj.seed.min\endcsname{0.38}
\expandafter\def\csname v@subj.xseed.max\endcsname{0.62}
\expandafter\def\csname v@subj.xseed.min\endcsname{0.49}
\makeatother

